One Model to Rule them all: Multitask and Multilingual Modelling for Lexical Analysis

When learning a new skill, you take advantage of your preexisting skills and knowledge. For instance, if you are a skilled violinist, you will likely have an easier time learning to play cello. Similarly, when learning a new language you take advantage of the languages you already speak. For instance, if your native language is Norwegian and you decide to learn Dutch, the lexical overlap between these two languages will likely benefit your rate of language acquisition. This thesis deals with the intersection of learning multiple tasks and learning multiple languages in the context of Natural Language Processing (NLP), which can be defined as the study of computational processing of human language. Although these two types of learning may seem different on the surface, we will see that they share many similarities. The traditional approach in NLP is to consider a single task for a single language at a time. However, recent advances allow for broadening this approach, by considering data for multiple tasks and languages simultaneously. This is an important approach to explore further as the key to improving the reliability of NLP, especially for low-resource languages, is to take advantage of all relevant data whenever possible. In doing so, the hope is that in the long term, low-resource languages can benefit from the advances made in NLP which are currently to a large extent reserved for high-resource languages. This, in turn, may then have positive consequences for, e.g., language preservation, as speakers of minority languages will have a lower degree of pressure to using high-resource languages. In the short term, answering the specific research questions posed should be of use to NLP researchers working towards the same goal.

==> backmatter/cv_english.tex <==
\chapter[Curriculum Vitae (English)]{Curriculum Vitae\\(English)}


==> backmatter/cv_nederlands.tex <==
\chapter{Curriculum Vitae (Nederlands)}


==> backmatter/grodil.tex <==
\chapter*{Groningen Dissertations in Linguistics (\textsc{Grodil})}
\markboth{GRODIL}{GRODIL}

\newcommand{\headrulewidth}{0.4pt}
\newcommand{\footrulewidth}{0pt}

\sloppy
\hyphenpenalty=10000
\begin{enumerate}
\setlength{\itemsep}{-0.5mm}
\footnotesize
\item Henri{\"e}tte de Swart (1991). \emph{Adverbs of Quantification: 
    A Generalized Quantifier Approach.} 
\item Eric Hoekstra (1991). \emph{Licensing Conditions on Phrase
    Structure.} 
\item Dicky Gilbers (1992). \emph{Phonological Networks. A Theory of
    Segment Representation.} 
\item Helen de Hoop (1992). \emph{Case Configuration and Noun Phrase
    Interpretation.} 
\item Gosse Bouma (1993). \emph{Nonmonotonicity and Categorial
    Unification Grammar.} 
\item Peter Blok (1993). \emph{The Interpretation of Focus: an
    epistemic approach to pragmatics.} 
\item Roelien Bastiaanse (1993). \emph{Studies in Aphasia.} 
\item Bert Bos (1993). \emph{Rapid User Interface Development with the
    Script Language Gist.} 
\item Wim Kosmeijer (1993). \emph{Barriers and Licensing.} 
\item Jan-Wouter Zwart (1993). \emph{Dutch Syntax: A Minimalist
    Approach.} 
\item Mark Kas (1993). \emph{Essays on Boolean Functions and Negative
    Polarity.} 
\item Ton van der Wouden (1994). \emph{Negative Contexts.} 
\item Joop Houtman (1994). \emph{Coordination and Constituency: A
    Study in Categorial Grammar.} 
\item Petra Hendriks (1995). \emph{Comparatives and Categorial
    Grammar.} 
\item Maarten de Wind (1995). \emph{Inversion in French.} 
\item Jelly Julia de Jong (1996). \emph{The Case of Bound Pronouns in
    Peripheral Romance.} 
\item Sjoukje van der Wal (1996). \emph{Negative Polarity Items and
    Negation: Tandem Acquisition.} 
\item Anastasia Giannakidou (1997). \emph{The Landscape of Polarity
    Items.} 
\item Karen Lattewitz (1997). \emph{Adjacency in Dutch and German.} 
\item Edith Kaan (1997). \emph{Processing Subject-Object Ambiguities
    in Dutch.} 
\item Henny Klein (1997). \emph{Adverbs of Degree in Dutch.} 
\item Leonie Bosveld-de Smet (1998). \emph{On Mass and Plural
    Quantification: The Case of French `des'/`du'-NPs.} 
\item Rita Landeweerd (1998). \emph{Discourse Semantics of Perspective
    and Temporal Structure.} 
\item Mettina Veenstra (1998). \emph{Formalizing the Minimalist
    Program.} 
\item Roel Jonkers (1998). \emph{Comprehension and Production of Verbs
    in Aphasic Speakers.} 
\item Erik F. Tjong Kim Sang (1998). \emph{Machine Learning of Phonotactics.} 
\item Paulien Rijkhoek (1998). \emph{On Degree Phrases and Result
    Clauses.} 
\item Jan de Jong (1999). \emph{Specific Language Impairment in Dutch:
    Inflectional Morphology and Argument Structure.} 
\item Hae-Kyung Wee (1999). \emph{Definite Focus.} 
\item Eun-Hee Lee (2000). \emph{Dynamic and Stative Information in
    Temporal Reasoning: Korean Tense and Aspect in Discourse.} 
\item Ivilin Stoianov (2001). \emph{Connectionist Lexical Processing.}
\item Klarien van der Linde (2001). \emph{Sonority Substitutions.} 
\item Monique Lamers (2001). \emph{Sentence Processing: Using
    Syntactic, Semantic, and Thematic Information.} 
\item Shalom Zuckerman (2001). \emph{The Acquisition of ``Optional''
    Movement.} 
\item Rob Koeling (2001). \emph{Dialogue-Based Disambiguation: Using
    Dialogue Status to Improve Speech Understanding.} 
\begin{sloppypar}
\item Esther Ruigendijk (2002). \emph{Case Assignment in Agrammatism: a
    Cross-linguistic Study.}
\end{sloppypar} 
\item Tony Mullen (2002). \emph{An Investigation into Compositional
    Features and Feature Merging for Maximum Entropy-Based Parse
    Selection.} 
\item Nanette Bienfait (2002). \emph{Grammatica-onderwijs aan
    allochtone jong\-eren.} 
\item Dirk-Bart den Ouden (2002). \emph{Phonology in Aphasia:
    Syllables and Segments in Level-specific Deficits.} 

\item Rienk Withaar (2002). \emph{The Role of the Phonological Loop in
    Sentence Comprehension.} 
\item Kim Sauter (2002). \emph{Transfer and Access to Universal
    Grammar in Adult Second Language Acquisition.} 
\item Laura Sabourin (2003). \emph{Grammatical Gender and Second
    Language Processing: An ERP Study.} 
\item Hein van Schie (2003). \emph{Visual Semantics.} 
\item Lilia Sch{\"u}rcks-Grozeva (2003). \emph{Binding and Bulgarian.}
\item Stasinos Konstantopoulos (2003). \emph{Using ILP to Learn Local
    Linguistic Structures.} 
\item Wilbert Heeringa (2004). \emph{Measuring Dialect Pronunciation
    Differences using Levenshtein Distance.} 
\item Wouter Jansen (2004). \emph{Laryngeal Contrast and Phonetic
    Voicing: A Laboratory Phonology Approach to English, Hungarian and
    Dutch.} 
\item Judith Rispens (2004). \emph{Syntactic and Phonological
    Processing in Developmental Dyslexia.} 
\item Danielle Bouga\"{\i}r\'e (2004). \emph{L'approche communicative
    des campagnes de sensibilisation en sant\'e publique au Burkina
    Faso: les cas de la planification familiale, du sida et de
    l'excision.} 
\item Tanja Gaustad (2004). \emph{Linguistic Knowledge and Word Sense
    Disambiguation.} 
\item Susanne Schoof (2004). \emph{An HPSG Account of Nonfinite Verbal
    Complements in Latin.}
\item M. Bego\~na Villada Moir\'on (2005). \emph{Data-driven identification of
fixed expressions and their modifiability.}
\item Robbert Prins (2005). \emph{Finite-State Pre-Processing for Natural
Language Analysis.}
\item Leonoor van der Beek (2005). \emph{Topics in Corpus-Based Dutch Syntax.}
\item Keiko Yoshioka (2005). \emph{Linguistic and gestural introduction and
tracking of referents in L1 and L2 discourse.}
\item Sible Andringa (2005). \emph{Form-focused instruction and the development
of second language proficiency.}
\item Joanneke Prenger (2005). \emph{Taal telt! Een onderzoek naar de rol van
taalvaardigheid en tekstbegrip in het realistisch wiskundeonderwijs.}
\item Neslihan Kansu-Yetkiner (2006). \emph{Blood, Shame and Fear:
Self-Presentation Strategies of Turkish Women's Talk about their Health and
Sexuality.}
\item M\'onika Z. Zempl\'eni (2006). \emph{Functional imaging of the hemispheric
contribution to language processing. }
\item Maartje Schreuder (2006). \emph{Prosodic Processes in Language and Music.}
\item Hidetoshi Shiraishi (2006). \emph{Topics in Nivkh Phonology.}
\item Tam\'as Bir\'o (2006). \emph{Finding the Right Words: Implementing
Optimality Theory with Simulated Annealing.}
\item Dieuwke de Goede (2006). \emph{Verbs in Spoken Sentence Processing:
Unraveling the Activation Pattern of the Matrix Verb.}
\item Eleonora Rossi (2007). \emph{Clitic production in Italian agrammatism.}
\item Holger Hopp (2007). \emph{Ultimate Attainment at the Interfaces in Second
Language Acquisition: Grammar and Processing. }
\item Gerlof Bouma (2008). \emph{Starting a Sentence in Dutch: A corpus study of
subject- and object-fronting. }
\item Julia Klitsch (2008). \emph{Open your eyes and listen carefully. Auditory
and audiovisual speech perception and the McGurk effect in Dutch speakers with
and without aphasia.}
\item Janneke ter Beek (2008). \emph{Restructuring and Infinitival Complements
in Dutch.}
\item Jori Mur (2008). \emph{Off-line Answer Extraction for Question
Answering.}
\item Lonneke van der Plas (2008). \emph{Automatic Lexico-Semantic
Acquisition for Question Answering.}
\item Arjen Versloot (2008). \emph{Mechanisms of Language Change: Vowel
reduction in 15th century West Frisian.}
\item Ismail Fahmi (2009). \emph{Automatic term and Relation Extraction for
Medical Question Answering System.}
\item Tuba Yarbay Duman (2009). \emph{Turkish Agrammatic Aphasia: Word Order,
Time Reference and Case.}
\item Maria Trofimova (2009). \emph{Case Assignment by Prepositions in Russian
Aphasia.}
\item Rasmus Steinkrauss (2009). \emph{Frequency and Function in WH Question
Acquisition. A Usage-Based Case Study of German L1 Acquisition.}
\item Marjolein Deunk (2009). \emph{Discourse Practices in Preschool. Young
Children's Participation in Everyday Classroom Activities.}
\item Sake Jager (2009). \emph{Towards ICT-Integrated Language Learning:
Developing an Implementation Framework in terms of Pedagogy, Technology and
Environment.}
\item Francisco Dellatorre Borges (2010). \emph{Parse Selection with Support
Vector Machines.}
\item Geoffrey Andogah (2010). \emph{Geographically Constrained Information
Retrieval.}
\item Jacqueline van Kruiningen (2010). \emph{Onderwijsontwerp als conversatie.
Probleemoplossing in interprofessioneel overleg.}
\item Robert G. Shackleton (2010). \emph{Quantitative Assessment of
English-American Speech Relationships.}
\item Tim Van de Cruys (2010). \emph{Mining for Meaning: The Extraction of
Lexico-semantic Knowledge from Text.}
\item Therese Leinonen (2010). \emph{An Acoustic Analysis of Vowel Pronunciation
in Swedish Dialects.}
\item Erik-Jan Smits (2010). \emph{Acquiring Quantification. How Children Use
Semantics and Pragmatics to Constrain Meaning.}
\item Tal Caspi (2010). \emph{A Dynamic Perspective on Second Language
Development.}
\item Teodora Mehotcheva (2010). \emph{After the fiesta is over. Foreign
language attrition of Spanish in Dutch and German Erasmus Students.}
\item Xiaoyan Xu (2010). \emph{English language attrition and retention in
Chinese and Dutch university students.}
\item Jelena Proki\'c (2010). \emph{Families and Resemblances.}
\item Radek \v{S}im\'ik (2011). \emph{Modal existential wh-constructions.}
\item Katrien Colman (2011). \emph{Behavioral and neuroimaging studies on
language processing in Dutch speakers with Parkinson's disease.}
\item Siti Mina Tamah (2011). \emph{A Study on Student Interaction in the
Implementation of the Jigsaw Technique in Language Teaching.}
\item Aletta Kwant (2011). \emph{Geraakt door prentenboeken. Effecten van het
gebruik van prentenboeken op de sociaal-emotionele ontwikkeling van kleuters.}
\item Marlies Kluck (2011). \emph{Sentence amalgamation.}
\item Anja Sch\"uppert (2011). \emph{Origin of asymmetry: Mutual intelligibility
of spoken Danish and Swedish.}
\item Peter Nabende (2011). \emph{Applying Dynamic Bayesian Networks in
Transliteration Detection and Generation.}
\item Barbara Plank (2011). \emph{Domain Adaptation for Parsing.}
\item \c{C}a\u{g}r{\i} \c{C}\"oltekin (2011). \emph{Catching Words in
a Stream of Speech: Computational simulations of segmenting transcribed child-directed speech.}
\item D\"orte Hessler (2011). \emph{Audiovisual Processing in Aphasic and Non-Brain-Damaged Listeners: 
The Whole is More than the Sum of its Parts.}
Herman Heringa (2012). \emph{Appositional constructions.}
\item Herman Heringa (2012). \emph{Appositional constructions.}
\item Diana Dimitrova (2012). \emph{Neural Correlates of Prosody and Information Structure.}
\item Harwintha Anjarningsih (2012). \emph{Time Reference in Standard Indonesian Agrammatic Aphasia.}
\item Myrte Gosen (2012). \emph{Tracing learning in interaction. An analysis of shared reading of picture books at kindergarten.}
\item Martijn Wieling (2012). \emph{A Quantitative Approach to Social and Geographical Dialect Variation.}
\item Gisi Cannizzaro (2012). \emph{Early word order and animacy.}
\item Kostadin Cholakov (2012). \emph{Lexical Acquisition for Computational Grammars. A Unified Model.}
\item Karin Beijering (2012). \emph{Expressions of epistemic modality in Mainland Scandinavian. A study into the lexicalization-grammaticalization-pragmaticalization interface.}
\item Veerle Baaijen (2012). \emph{The development of understanding through writing.}
\item Jacolien van Rij (2012). \emph{Pronoun processing: Computational, behavioral, and psychophysiological studies in children and adults.}
\item Ankelien Schippers (2012). \emph{Variation and change in Germanic long-distance dependencies.}
\item Hanneke Loerts (2012). \emph{Uncommon gender: Eyes and brains, native and second language learners, \& grammatical gender.}
\item Marjoleine Sloos (2013). \emph{Frequency and phonological grammar: An integrated approach. Evidence from German, Indonesian, and Japanese.}
\item Aysa Arylova (2013). \emph{Possession in the Russian clause. Towards dynamicity in syntax.}
\item Dani\"el de Kok (2013). \emph{Reversible Stochastic Attribute-Value
Grammars.}
\item Gideon Kotz\'e (2013). \emph{Complementary approaches to tree
alignment: Combining statistical and rule-based methods.}
\item Fridah Katushemererwe (2013). \emph{Computational Morphology and Bantu
Language Learning: an Implementation for Runyakitara.}
\item Ryan C. Taylor (2013). \emph{Tracking Referents: Markedness, World
Knowledge and Pronoun Resolution.}
\item Hana Smiskova-Gustafsson (2013). \emph{Chunks in L2 Development:
A Usage-Based Perspective.}
\item Milada Walkov\'a (2013). \emph{The aspectual function of particles in
phrasal verbs.}
\item Tom O. Abuom (2013). \emph{Verb and Word Order Deficits in
Swahili-English bilingual agrammatic speakers.}
\item G\"ulsen Y{\i}lmaz (2013). \emph{Bilingual Language Development among the
First Generation Turkish Immigrants in the Netherlands.}
\item Trevor Benjamin (2013). \emph{Signaling Trouble: On the linguistic
design of other-initiation of repair in English Conversation.}
\item Nguyen Hong Thi Phuong (2013). \emph{A Dynamic Usage-based Approach to
Second Language Teaching.}
\item Harm Brouwer (2014). \emph{The Electrophysiology of Language Comprehension:
A Neurocomputational Model.}
\end{enumerate}

\bigskip

\noindent
\textsc{Grodil} \\
Secretary of the Department of General Linguistics\\
Postbus 716\\
9700 AS Groningen\\
The Netherlands


==> backmatter/publications.tex <==
\chapter{List of Publications}

\begin{enumerate}

        \item %\bibentry{venhuizen2014how}

        \item %\bibentry{hoeks2014electrophysiological}

        \item %\bibentry{brouwer2013time}

        \item %\bibentry{hoeks2013questions}

        \item %\bibentry{venhuizen2013parsimonious}

        \item %\bibentry{brouwer2012getting}

        \item %\bibentry{brouwer2010modeling}

\end{enumerate}


==> comp_sem/dataset_augmentation.tex <==
\renewcommand*{\thefootnote}{\fnsymbol{footnote}}
\chapter[Dataset Augmentation]{\footnote{Chapter adapted from: \textbf{Bjerva, J.} (in prep) \textit{Improving Semantic Classification with Dataset Augmentation} | and \textbf{Bjerva, J.} (2014) \textit{Animacy Classification with Semantic Features}}
\hspace{-6pt}Dataset Augmentation for\\Semantic Classification\hspace{-8pt}}

\renewcommand*{\thefootnote}{\arabic{footnote}}

\todo[inline]{Maybe rename to something like 'alternative approaches to MTL?'}

\label{chp:data_aug}
\label{chp:dataset_aug}
\input{comp_sem/dataset_augmentation_text}


==> comp_sem/dataset_augmentation_bu.tex <==
\renewcommand*{\thefootnote}{\fnsymbol{footnote}}
\chapter[Dataset Augmentation]{Dataset Augmentation\footnote{Chapter adapted from: Bjerva, J. and Bos, J. (in prep.)}}
% Linguistic dataset augmentation improves semantic classification in Transactions of the Association for Computational Linguistics, x:ppp-ppp}}
\renewcommand*{\thefootnote}{\arabic{footnote}}

\begin{abstract}
The simplest way of increasing the generalisation ability of a machine learning model is to provide it with more training data.
However, the availability of tagged training data is often limited, and creating more human annotated data is expensive.
In this paper we show how automatic dataset augmentation can be applied to NLP, thus increasing system performance quickly and at no cost.
We adapt this to several noun compound classification tasks and datasets, and achieve state-of-the-art performances on all of these.
%, reducing error rates by more than 5\% for one dataset.
We outperform previous systems which use complex features and learning architectures, using a simple neural network architecture with off-the-shelf word embedding features, coupled with augmented datasets.
%More complex features and task-specific embeddings are expected to further improve upon the gains obtained from our method.
\end{abstract}

\section{Introduction}

The most straightforward way to make a machine learning model generalise better is to provide it with more training data.
In practice, however, the amount of data available is far from infinite, and creating more human annotated data is both time-consuming and expensive.
To get around this problem, one can create more fake data by dataset augmentation, i.e., by altering the original data in relatively minor ways so as to produce new training examples.
For many tasks this is reasonably simple.
Within the setting of computer vision, this is frequently done by scaling and rotating input images.
Since a given image can be scaled and rotated in many imaginable ways, datasets can be made much larger with relatively little effort.
Care must be taken not to apply transformations that are relevant to the problem at hand, however.
For example, optical character recognition requires there to be a difference between \textit{b, p, d} and \textit{q}, so horizontal flips and 180 degree rotations are not appropriate ways of augmenting this data.

In the case of NLP, applying geometric transformations to atomic units such as words does not seem quite as straightforward.
Ideally one would want to generate new augmented training examples which are similar to the original training data, while maintaining as much information as possible in a way such that the label of the original training example is also applicable to the augmented training example.
The advantage of having a general dataset augmentation method for NLP is that one could potentially increase performance for a large number of NLP tasks.
This will, in turn, increase the performance of higher level tasks such as machine translation.

In this paper we investigate how dataset augmentation can be adapted to several NLP datasets for semantic classification tasks.
We investigate which of two lexical resources, one manually created and one automatically generated, is the most suited for this task.
We report on experiments on four annotated noun compound datasets \citep{Tratz:2011,Oseaghdha:2008,KimBaldwin:2005,Bos:2015} using the Paraphrase Database \citep{ppdb} and WordNet \citep{Miller:1995} for dataset augmentation by replacing constituents in each compound with (near) synonyms.
We use a simple neural network learning architecture with features from off-the-shelf word embeddings so as to highlight the advantage of applying dataset augmentation.

The rest of this paper is structured as follows:
Section 2 presents related work on noun compound interpretation and dataset augmentation.
Section 3 outlines the datasets and lexical resources used in this work.
Section 4 describes the method.
In Section 5 we present our results.
Section 6 contains a discussion, and we conclude in Section 7.

\section{Related work}

\subsection{Noun Compound Interpretation}

The task of Noun Compound interpretation has long been the subject of research efforts.
In addition to attempts at improving classification scores on this task, a large amount of datasets have been made, with various annotation schemes.
One of the earliest approaches is presented by \citet{Lauer:1995}.
\citet{RosarioHearst:2001} attempt domain-specific noun compound relation classification, using medical texts.
\citet{KimBaldwin:2005} present a new dataset with classification experiments based on calculating similarities between instances in the training and test set.
\citet{Girju:2005} use WordNet-based models and SVMs to classify noun compounds consisting of two and three words.
\citet{Oseaghdha:2008} presents a dataset, and \citet{OseaghdhaCopestake:2013} report the current state-of-the-art experiments on this dataset.
\citet{TratzHovy:2010} present a dataset and experiments, and \citet{Tratz:2011} refines this dataset.
\citet{DimaHinrichs:2015} present the current state-of-the-art experiments on the Tratz dataset \citep{Tratz:2011}.
\citet{Bos:2015} present a dataset annotated via crowdsourcing.
All of the aforementioned efforts focus on English.
As for other languages, \citet{Verhoeven:2012} report experiments for Dutch and Afrikaans.

We contribute to previous work on noun compound interpretation by experimenting on and improving classification accuracy on several such datasets.

\subsection{Dataset Augmentation}
\label{sec:dataset_augmentation_background}

For many machine learning methods, and particularly for deep learning, appropriate dataset augmentation techniques are important to increase the generalisation ability of a model.
Such techniques work well when invariant properties which the model should posess are manipulated.
For instance, in image recognition, a model should have invariance towards changes such as scaling and rotation (see e.g. \citet{Duin:1997,Tompson:2014}).
In speech recognition, data is often augmented by adding training examples with artificial background noise, or with the speed or tone of the speech signal altered \citep{Hannun:2014}.
The advantages of dataset augmentation lie not only in the increased data set sizes, but also in the fact that adding such noisy input can increase the robustness of the model learned by a neural network.
This is due to the fact that the model is forced to learn a representation which is invariant to this added noise, which is especially relevant in the case of neural networks, as they are not particularly robust to noise \citep{TangEliasmith:2010}.

In natural language processing, however, dataset augmentation is more finicky, as simple signal manipulation methods are not as feasible.
One option is to increase training data sizes by manually rephrasing sentences.
\citet{DeVault:2011} show that expanding training data in this manner does improve results for dialogue systems.
However, as this is both expensive and time-consuming, a data-driven method of augmenting natural language data is needed.
\citet{Gardent:2013} build upon this by automatically generating paraphrases using a pivoting translation approach with Google Translate, resulting in increased performance in a QA system.
Their approach has the drawback that it is both relatively complex, and that reproducing their work would be challenging as the ever-changing online blackbox of GT is used.
\citet{Zhang:2015} present experiments on text understanding, in which they make attempts at manipulating a dataset using a thesaurus obtained indirectly from WordNet \citep{Fellbaum:2005} via the LibreOffice project.
Replaceable words are extracted from a given text, and a random subset of these are replaced with a synonym.
However, they note that with their already large dataset sizes, dataset augmentation does not have much impact.
A small increase in testing accuracy is obtained using their dataset augmentation method (98.3\% accuracy without augmentation, 98.4\% accuracy with augmentation).

Dataset augmentation for NLP consists of a very small body of work, and is in need of more attention.
We contribute to previous work by showing how such a method can be adapted to noun compound classification.
We compare two popular lexical resources and show which offers the best performance in our experimental setting.
We compare using both na\"ive and linguistically informed dataset augmentation methods.
We show that substantial gains in classification accuracy can be achieved using a simple dataset augmentation procedure, highlighting the need of more research in this area.


\section{Datasets and Lexical Resources}
We experiment on four annotated noun compound datasets.
An overview of these datasets is shown in Table~\ref{tab:datasets}.

\setlength{\tabcolsep}{6pt}
\begin{table}[h]
\centering
\caption{\label{tab:datasets}Overview of the datasets used in this study.}
\begin{tabular}{lrr}
\hline
{\bf Dataset} & {\bf Compounds } & {\bf Relations} \\
\hline
{\it Tratz}          & 19158 & 37 \\
{\it \oshay}         & 1443  & 6 / 11 / 37\\
{\it Kim \& Baldwin} & 2169  & 20 \\
{\it Wordrobe}       & 965   & 25 \\
\hline
\end{tabular}
\end{table}

\subsection{Tratz dataset}

The Tratz dataset \citep{Tratz:2011} is the largest annotated noun compound dataset which is publicly available, containing 19,158 compounds annotated with 37 semantic relations.\footnote{Tratz: \url{isi.edu/publications/licensed-sw/fanseparser/}}
The inventory of relations consists of semantic categories resembling those previously proposed by \citet{Barker:1998} and \citet{Girju:2005}.
The altered inventory of relations, as compared to \citet{Barker:1998}, is motivated by \citet{TratzHovy:2010} by the resulting increased inter-annotator agreement.
Furthermore, \citet{Tratz:2011} motivate the revision of relations by the necessity of creating a better mapping between prepositional paraphrases and noun compound relations.
The state-of-the-art results on this dataset are in the range 77.12\% - 79.38\% \citep{DimaHinrichs:2015}.

\subsection{\oshay dataset}

The \oshay dataset is a much smaller annotated noun compound dataset, containing 1,443 compounds annotated with semantic relations at three levels of granularity \citep{Oseaghdha:2008}.\footnote{{\'O} S{\'e}aghdha: \url{cl.cam.ac.uk/~do242/Resources/}}
The annotated relations can be summed up as follows:
\begin{itemize}
  \item Coarse: \textsc{be}, \textsc{have}, \textsc{in}, \textsc{actor}, \textsc{instrument}, \textsc{about} (6 labels);
  \item Directed: coarse relations with directionality (11 labels);
  \item Fine: fine-grained labels corresponding to annotation rules and which constituents fill which relation slots (37 labels).
\end{itemize}
The state-of-the-art results on this dataset are 65.4\% (Coarse), 65.1\% (Directed) and 53.9\% (Fine) \citep{OseaghdhaCopestake:2013}.

\subsection{Kim \& Baldwin dataset}

The Kim \& Baldwin dataset is another small annotated noun compound dataset, containing 2169 compounds annotated with 20 labels \citep{KimBaldwin:2005}.\footnote{Kim \& Baldwin: \url{multiword.sourceforge.net}}
This dataset notably has a low inter-annotator agreement of 52.3\%, and relatively unevenly distributed data \citep{TratzHovy:2010}.
The state-of-the-art result on this dataset is 53.3\% \citep{KimBaldwin:2005}.

\setlength{\tabcolsep}{6pt}
\begin{table*}[t]
\footnotesize
\centering
\caption{\label{tab:augment_examples}Randomly chosen examples of augmented compounds with one replaced constituent using both WordNet conditions and all PPDB sizes, with the source compound and its annotated relation group in the Tratz dataset \citep{Tratz:2011}.}
\begin{tabular}{llllll}
  \hline
  {\bf Relation} & \textsc{complement} & \textsc{topic} & \textsc{objective} & \textsc{measure} & \textsc{purpose} \\
  \hline
  {\bf Original} & family background & arms talk & gold dealer & miles km & care center \\
  {\bf WN first} & menage background & munition talk & gold bargainer & miles klick & tending center \\
  {\bf WN all} & fellowship background & blazon talk & u dealer & knot km & forethought center \\
  {\bf PPDB S} & families background & weapons talk & gold concessionaire & miles kilometres & care centre \\
  {\bf PPDB M} & family context & armaments talk & gold distributor & km km & attention center \\
  {\bf PPDB L} & household background & arm talk & kim dealer & thousands km & caring center \\
  {\bf PPDB XL} & familia background & weaponry talk & dorado dealer & kilometers km & soins center \\
  {\bf PPDB XXL} & range background & booby talk & air dealer & mi km & saves center \\
  {\bf PPDB XXXL} & genealogy background & utensils talk & thumb dealer & millions km & payload center \\
\hline
\end{tabular}
\end{table*}

\subsection{Noun-Noun Compounds from Gamification}
\citet{Bos:2015} describe a gamification-based method for obtaining noun-noun compound annotations.
Wordrobe \citep{wordrobe} is used in order to tag noun-noun compounds with relations based on 26 prepositions.
Overall, 25 of these are used by the annotators on a dataset containing 965 compounds.\footnote{Wordrobe: \url{gmb.let.rug.nl/data.php}}
To the best of our knowledge, there is no previous work reporting classification accuracies on this dataset.

\subsection{The Paraphrase Database}
The Paraphrase Database (PPDB) is a collection of paraphrases which has been automatically constructed using bilingual pivoting \citep{ppdb}.
This resource includes paraphrases of lexical units as well as longer phrases, and exists in six sizes following a continuum from highest precision and lowest recall, to lowest precision and highest recall (S, M, L, XL, XXL, XXXL).
The smallest versions (S, M) contain a large proportion of equivalent paraphrases, whereas larger versions (L, XL) increasingly contain paraphrases which entail each other, and the largest versions (XXL, XXXL) contain a large amount of otherwise related or independent paraphrases \citep{PavlickBosEtAl:2015}.

The recently released PPDB 2.0 adds to the original PPDB by reranking paraphrases in a better way as judged by humans, as well as including explicit entailment relations between paraphrases, style classification and distances obtained from a word embedding model \citep{ppdb2}.
The entailment relations used are: equivalence, forward/reverse entailment, opposites, independent, and other \citep{PavlickBosEtAl:2015}.

\subsection{WordNet}
WordNet is a manually created lexical resource in which words are grouped into groups of synonyms called synsets \citep{Miller:1995,Fellbaum:2005}.
Synonyms of a given word can be looked up by, e.g., retrieving the most common sense of that word in WordNet and extracting all lemmas of that synset, or by extracting all lemmas of all synsets to which a word belongs.
We use WordNet version 3.0 in our experiments.

\section{Method}

\subsection{Dataset Augmentation for NLP}
We use a prelease of PPDB 2.0 as a source of synonyms and near-synonyms, drawn from its available lexical paraphrase packs.\footnote{PPDB 2.0: \url{seas.upenn.edu/~epavlick/data.html}}
Since we are experimenting with datasets consisting of noun compounds, we only use a subset of PPDB filtered to contain only nominal paraphrases.
This is done based on the constituent tag available for each paraphrase in the PPDB.
Experiments are run using all sizes of the PPDB (S, M, L, XL, XXL, XXXL).

We also experiment using WordNet 3.0 as a source of synonyms and near-synonyms.
We extract these in two ways.
In the \textsc{wn first} setting, we use all lemmas of the most frequent sense of the given word.
In the \textsc{wn all} setting, we use all lemmas of \textit{all} senses of the given word.

Our dataset augmentation procedure is as follows.
Every noun compound (e.g. \textit{dog house}) in the training sets is split into its two constituents (e.g. \textit{dog} and \textit{house}).
We generate new augmented noun compounds in two ways. In one setting, \textsc{unigram}, we keep one constituent constant (e.g. \textit{dog}), while replacing the other (e.g. \textit{house}) with available synonyms and near-synonyms (e.g. \textit{home}, \textit{chamber}).
We generate augmented examples in which the first constituent is changed as well as ones where the second constituent is changed.
In the second setting, \textsc{bigram}, we replace both constituents of the compound with a bigram paraphrase from PPDB or with two unigram paraphrases from WordNet.
\todo[inline]{Choice made since WordNet does not contain (many) bigrams?}
We also combine these two approaches, in a \textsc{unigram+bigram} setting.
The results of this procedure is a much larger and inflated list of compounds (e.g. \textit{dog home}, \textit{canine house}, \textit{hound home}).
Note that the original compounds are also kept in the training set.
Although the augmented compounds, such as listed above, represent somewhat awkward or non-natural phrasings of the compound \textit{dog house}, they convey the same relation as the original compound.
That is to say, both \textit{dog house} and \textit{canine house} should be labelled \textsc{user-recipient} if following the annotation scheme in \citet{Tratz:2011}.
Randomly chosen examples of augmented compounds with one replaced constituent are shown in Table~\ref{tab:augment_examples} with the original compound and its relation group in the Tratz dataset.

Performing this dataset augmentation process yields new training data sizes as shown in Figure~\ref{fig:data_augment}.
Depending on the source of (near) synonyms, the new training sets are scaled from as little as 1.5 times to as much as almost 1000 times.
The smallest augmented datasets thus contain a minority of augmented examples, whereas original examples are massively outnumbered in the largest augmented datasets.

\begin{figure}[h]
  \centering
  %\includegraphics[width=0.5\textwidth]{./data_sizes.png}
  \missingfigure{data sizes}
  \caption{\label{fig:data_augment}Proportion of augmented data per condition. The y-axis shows data set size increase on a log scale.}
\end{figure}

We considered controlling the augmentation process by asserting that we do not include data which are identical to ones in the dev and test sets, by disallowing compounds which occur in these sets to be included in the dataset augmentation process.
The experiments reported in this paper do not make this assertion.
Considering that the test set should be completely unknown at development time, such an assertion would be unrealistic.
Furthermore, such a control would perhaps unfairly put our method at an advantage.
Preliminary experiments showed that whether or not this was controlled for had very little impact on results on the development set.

\subsection{Dataset pre-processing}
We use the same simple pre-processing step for all datasets, consisting of converting all words to lower case.
This is necessary since the embeddings we use are trained on lower-cased text, whereas several of the datasets contain words with upper-case letters (e.g. proper nouns in the Tratz dataset).

\subsection{Evaluation}
For the Kim \& Baldwin dataset we use the official training / testing splits, and use 10\% of the training data as development data.
For all other datasets, the data is randomly shuffled and split into 20\% / 10\% / 70\% for testing, development and training respectively.
We use the combined training and development splits to construct 5-fold cross-validation sets.

The overall best PPDB condition and WordNet condition is chosen based on the results on the development sets.
We report test set accuracies using these two conditions.

\begin{figure*}[ht]
    \centering
  %  \subfigure[WN]{\includegraphics[width=0.49\textwidth]{./wordnet_xval.png}}
  %  \subfigure[PPDB]{\includegraphics[width=0.49\textwidth]{./ppdb_xval.png}}
    \missingfigure{Figure here.}
    \caption{\label{fig:xval}WN and PPDB xval scores. Dashed lines represent previous state-of-the-art results for each dataset. (PLACEHOLDER FIGURES).}
\end{figure*}

\begin{figure*}[ht]
  \centering
  \include{neural_network}
  \caption{\label{fig:nn}Neural network architecture used in our experiments. Each layer has $n=600$ units, except for the output layer with $n=k$ units whrere $k$ is the amount of semantic relations to classify for the given dataset. The inputs are given by mapping both nouns in each given compound to their vectors in the word embeddings used, and concatenating these.}
\end{figure*}

\subsection{Features}
We use two types of features in our experiments: word embeddings and entailment relations obtained from PPDB 2.0.

Continuous space representations of words are currently the backbone of several state-of-the-art approaches to problems in natural language processing.
The distributional hypothesis, summarised as: `You shall know a word by the company it keeps' \citep{firth} is the basis of many approaches for obtaining such representations.
Word embeddings are an example of such a model (e.g. \citet{collobert:2008}), and have been found to encapsulate interesting semantic properties; in a model presented by \citet{Mikolov:13:Regularities}, the result when calculating
\mbox{$\overrightarrow{\textsc{king}} - \overrightarrow{\textsc{man}}
+ \overrightarrow{\textsc{woman}}$},
is close to $\overrightarrow{\textsc{queen}}$.
Although the seemingly magical properties of the Mikolov embeddings have been disspelled (cf. \citet{Levy:2015}), they perform remarkably well.\todo{This paragraph is perhaps a bit TMI.}

In this work we use publicly available embeddings, with 300 dimensions, which have been pre-trained on about 100 billion words.\footnote{Embeddings: \url{code.google.com/p/word2vec/}}
This choice was made so as to facilitate reproducibility of our work.
However, previous work has highlighted the importance of parameter selection in word embeddings (cf. \citet{Tang:2014,Levy:2015}), and we therefore expect there to be further room for improvement to the scores reported in this paper when using embeddings tuned to the task at hand.

The entailment relations obtained from PPDB 2.0 are used as an extra feature in the experiments which employ this resource.
For each augmented training example, a feature vector with one-hot encoding is concatenated to the standard feature vector.
Original examples in the training, development and test sets thus contain zero values in each of these extra feature dimensions.

\subsection{Experimental setting}
We use a simple feed-forward neural network in our classification experiments, implemented in Theano \citep{theano:orig,theano:nips} and Keras.\footnote{Keras: \url{http://keras.io/}}
We use a single hidden layer, with the same amount of neurons as the input layer (how many)\todo{how many}.
We use the ADAM optimisation algorithm \citep{Kingma:2014}.
We use maxout, which effectively learns the most appropriate activation function of each neuron \citep{maxout}.\todo{output layer}
\todo[inline]{Cost function, batch-size, learning rate}
\todo[inline]{Initialization}
Maxout can be advantageous compared to popular Rectified Linear Units (ReLUs), since ReLUs can get stuck by learning to de-activate and never again be re-activated \citep{rectifier,maxout}.
We employ dropout as regularisation \citep{dropout}. This essentially entails randomly forgetting a certain proportion of neurons after each epoch, which encourages neurons not to be dependent on the values of other neurons (since they can and do disappear at any time), thus increasing the robustness and generalisation ability of the neural network.
All hyper-parameters except for dropout probabilities are kept constant in all conditions and for all datasets.
We vary dropout probabilities in the range $[p=0.1,p=0.5]$ for the input layer and $[p=0.3,p=0.8]$ for the hidden layer.
The best performing parameter setting is reported in Table~\ref{tab:dropout_prob}, as judged per condition per development set.

\begin{table*}[h]
\small
\centering
\caption{\label{tab:dropout_prob}Dropout probabilities (input, hidden) as tuned on each development set and condition.}
\begin{tabular}{lrrrrrr}
  \hline
   & {\it Tratz} & {\it \oshay Coarse} & {\it \oshay Directed} & {\it \oshay Fine} & {\it Kim\&Baldwin}  & {\it Wordrobe}\\
  \hline
  {\it o} &&&&&&\\% $0.596 (\pm0.013)$ & $0.604 (\pm0.021)$ & $0.491 (\pm0.014)$ & $0.803 (\pm0.003)$ & $0.472 (\pm0.009)$\\
  {\it wn\_first} &&&&&&\\% $0.755 (\pm0.019)$ & $0.760 (\pm0.019)$ & $0.696 (\pm0.016)$ & $0.851 (\pm0.002)$ & $0.739 (\pm0.019)$\\
  {\it wn\_all} &&&&&&\\% $0.816 (\pm0.013)$ & $0.814 (\pm0.011)$ & $0.773 (\pm0.009)$ & $0.851 (\pm0.003)$ & $0.729 (\pm0.018)$\\
  {\it s} &&&&&&\\% $0.683 (\pm0.016)$ & $0.688 (\pm0.026)$ & $0.600 (\pm0.012)$ & $0.832 (\pm0.004)$ & $0.630 (\pm0.022)$\\
  {\it m} &&&&&&\\% $0.733 (\pm0.014)$ & $0.725 (\pm0.007)$ & $0.676 (\pm0.008)$ & $0.842 (\pm0.003)$ & $0.658 (\pm0.008)$\\
  {\it l} &&&&&&\\% $0.852 (\pm0.010)$ & $0.851 (\pm0.012)$ & $0.816 (\pm0.010)$ & $0.889 (\pm0.001)$ & $0.805 (\pm0.008)$\\
  {\it xl} &&&&&&\\% $0.865 (\pm0.010)$ & $0.857 (\pm0.011)$ & $0.815 (\pm0.011)$ & $0.900 (\pm0.003)$ & $0.811 (\pm0.016)$\\
  {\it xxl} &&&&&&\\% $0.858 (\pm0.012)$ & $0.841 (\pm0.012)$ & $0.809 (\pm0.007)$ & $0.894 (\pm0.002)$ & $0.817 (\pm0.009)$\\
  {\it xxxl} &&&&&&\\% $0.850 (\pm0.010)$ & $0.834 (\pm0.011)$ & $0.797 (\pm0.007)$ & $0.837 (\pm0.002)$ & $0.808 (\pm0.007)$\\
\hline
\end{tabular}
\end{table*}

The input to our neural network consists of the concatenation of the embedded representations of both words in the noun compound at hand.
In the experiments where PPDB 2.0 is used, we also include the one-hot representation for the entailment relations of each augmented training example.
We train over the course of 500 epochs, using early stopping while monitoring performance on the development set at hand.
After one pass over only the training set, the development data is added to the training set and training runs until the previously best performing epoch, following \citet{BengioBook}.
The resulting test set accuracy is then reported.
The architecture used is illustrated in Figure~\ref{fig:nn}.

\setlength{\tabcolsep}{6pt}
\begin{table*}[t]
\small
\centering
\caption{\label{tab:unigram_dev_results}Cross-validation accuracies for all datasets under the \textsc{unigram} condition. Brackets contain standard error across the five folds used.}

\begin{tabular}{lrrrrrr}
  \hline
   & {\it Tratz} & {\it \oshay Coarse} & {\it \oshay Directed} & {\it \oshay Fine} & {\it Kim\&Baldwin}  & {\it Wordrobe}\\
  \hline
  {\it o} &&&&&&\\% $0.596 (\pm0.013)$ & $0.604 (\pm0.021)$ & $0.491 (\pm0.014)$ & $0.803 (\pm0.003)$ & $0.472 (\pm0.009)$\\
  {\it wn\_first} &&&&&&\\% $0.755 (\pm0.019)$ & $0.760 (\pm0.019)$ & $0.696 (\pm0.016)$ & $0.851 (\pm0.002)$ & $0.739 (\pm0.019)$\\
  {\it wn\_all} &&&&&&\\% $0.816 (\pm0.013)$ & $0.814 (\pm0.011)$ & $0.773 (\pm0.009)$ & $0.851 (\pm0.003)$ & $0.729 (\pm0.018)$\\
  {\it s} &&&&&&\\% $0.683 (\pm0.016)$ & $0.688 (\pm0.026)$ & $0.600 (\pm0.012)$ & $0.832 (\pm0.004)$ & $0.630 (\pm0.022)$\\
  {\it m} &&&&&&\\% $0.733 (\pm0.014)$ & $0.725 (\pm0.007)$ & $0.676 (\pm0.008)$ & $0.842 (\pm0.003)$ & $0.658 (\pm0.008)$\\
  {\it l} &&&&&&\\% $0.852 (\pm0.010)$ & $0.851 (\pm0.012)$ & $0.816 (\pm0.010)$ & $0.889 (\pm0.001)$ & $0.805 (\pm0.008)$\\
  {\it xl} &&&&&&\\% $0.865 (\pm0.010)$ & $0.857 (\pm0.011)$ & $0.815 (\pm0.011)$ & $0.900 (\pm0.003)$ & $0.811 (\pm0.016)$\\
  {\it xxl} &&&&&&\\% $0.858 (\pm0.012)$ & $0.841 (\pm0.012)$ & $0.809 (\pm0.007)$ & $0.894 (\pm0.002)$ & $0.817 (\pm0.009)$\\
  {\it xxxl} &&&&&&\\% $0.850 (\pm0.010)$ & $0.834 (\pm0.011)$ & $0.797 (\pm0.007)$ & $0.837 (\pm0.002)$ & $0.808 (\pm0.007)$\\
\hline
\end{tabular}
\end{table*}

\begin{table*}[t]
\small
\centering
\caption{\label{tab:bigram_dev_results}Cross-validation accuracies for all datasets under  the \textsc{bigram} condition. Brackets contain standard error across the five folds used.}

\begin{tabular}{lrrrrrr}
  \hline
   & {\it Tratz} & {\it \oshay Coarse} & {\it \oshay Directed} & {\it \oshay Fine} & {\it Kim\&Baldwin}  & {\it Wordrobe}\\
  \hline
  {\it o} &&&&&&\\% $0.596 (\pm0.013)$ & $0.604 (\pm0.021)$ & $0.491 (\pm0.014)$ & $0.803 (\pm0.003)$ & $0.472 (\pm0.009)$\\
  {\it wn\_first} &&&&&&\\% $0.755 (\pm0.019)$ & $0.760 (\pm0.019)$ & $0.696 (\pm0.016)$ & $0.851 (\pm0.002)$ & $0.739 (\pm0.019)$\\
  {\it wn\_all} &&&&&&\\% $0.816 (\pm0.013)$ & $0.814 (\pm0.011)$ & $0.773 (\pm0.009)$ & $0.851 (\pm0.003)$ & $0.729 (\pm0.018)$\\
  {\it s} &&&&&&\\% $0.683 (\pm0.016)$ & $0.688 (\pm0.026)$ & $0.600 (\pm0.012)$ & $0.832 (\pm0.004)$ & $0.630 (\pm0.022)$\\
  {\it m} &&&&&&\\% $0.733 (\pm0.014)$ & $0.725 (\pm0.007)$ & $0.676 (\pm0.008)$ & $0.842 (\pm0.003)$ & $0.658 (\pm0.008)$\\
  {\it l} &&&&&&\\% $0.852 (\pm0.010)$ & $0.851 (\pm0.012)$ & $0.816 (\pm0.010)$ & $0.889 (\pm0.001)$ & $0.805 (\pm0.008)$\\
  {\it xl} &&&&&&\\% $0.865 (\pm0.010)$ & $0.857 (\pm0.011)$ & $0.815 (\pm0.011)$ & $0.900 (\pm0.003)$ & $0.811 (\pm0.016)$\\
  {\it xxl} &&&&&&\\% $0.858 (\pm0.012)$ & $0.841 (\pm0.012)$ & $0.809 (\pm0.007)$ & $0.894 (\pm0.002)$ & $0.817 (\pm0.009)$\\
  {\it xxxl} &&&&&&\\% $0.850 (\pm0.010)$ & $0.834 (\pm0.011)$ & $0.797 (\pm0.007)$ & $0.837 (\pm0.002)$ & $0.808 (\pm0.007)$\\
\hline
\end{tabular}
\end{table*}

\begin{table*}[t]
\small
\centering
\caption{\label{tab:both_dev_results}Cross-validation accuracies for all datasets under the \textsc{unigram+bigram} condition. Brackets contain standard error across the five folds used.}

\begin{tabular}{lrrrrrr}
  \hline
   & {\it Tratz} & {\it \oshay Coarse} & {\it \oshay Directed} & {\it \oshay Fine} & {\it Kim\&Baldwin}  & {\it Wordrobe}\\
  \hline
  {\it o} &&&&&&\\% $0.596 (\pm0.013)$ & $0.604 (\pm0.021)$ & $0.491 (\pm0.014)$ & $0.803 (\pm0.003)$ & $0.472 (\pm0.009)$\\
  {\it wn\_first} &&&&&&\\% $0.755 (\pm0.019)$ & $0.760 (\pm0.019)$ & $0.696 (\pm0.016)$ & $0.851 (\pm0.002)$ & $0.739 (\pm0.019)$\\
  {\it wn\_all} &&&&&&\\% $0.816 (\pm0.013)$ & $0.814 (\pm0.011)$ & $0.773 (\pm0.009)$ & $0.851 (\pm0.003)$ & $0.729 (\pm0.018)$\\
  {\it s} &&&&&&\\% $0.683 (\pm0.016)$ & $0.688 (\pm0.026)$ & $0.600 (\pm0.012)$ & $0.832 (\pm0.004)$ & $0.630 (\pm0.022)$\\
  {\it m} &&&&&&\\% $0.733 (\pm0.014)$ & $0.725 (\pm0.007)$ & $0.676 (\pm0.008)$ & $0.842 (\pm0.003)$ & $0.658 (\pm0.008)$\\
  {\it l} &&&&&&\\% $0.852 (\pm0.010)$ & $0.851 (\pm0.012)$ & $0.816 (\pm0.010)$ & $0.889 (\pm0.001)$ & $0.805 (\pm0.008)$\\
  {\it xl} &&&&&&\\% $0.865 (\pm0.010)$ & $0.857 (\pm0.011)$ & $0.815 (\pm0.011)$ & $0.900 (\pm0.003)$ & $0.811 (\pm0.016)$\\
  {\it xxl} &&&&&&\\% $0.858 (\pm0.012)$ & $0.841 (\pm0.012)$ & $0.809 (\pm0.007)$ & $0.894 (\pm0.002)$ & $0.817 (\pm0.009)$\\
  {\it xxxl} &&&&&&\\% $0.850 (\pm0.010)$ & $0.834 (\pm0.011)$ & $0.797 (\pm0.007)$ & $0.837 (\pm0.002)$ & $0.808 (\pm0.007)$\\
\hline
\end{tabular}
\end{table*}

\section{Results}
Figure~\ref{fig:xval} shows the effect of the the WordNet and PPDB conditions used for dataset augmentation on classification accuracy using 5-fold cross validation on all datasets.
Table~\ref{tab:unigram_dev_results} contains dev set accuracies under the \textsc{unigram} condition, Table~\ref{tab:bigram_dev_results} contains dev set accuracies under the \textsc{bigram} condition, and Table~\ref{tab:both_dev_results} contains dev set accuracies under the \textsc{unigram+bigram} condition.
The XXX condition yields better results in most cases.
Within this condition, using the PPDB size L provides the best results, with even larger sizes yielding slightly lower results.
Dataset augmentation improves performance on all datasets, both as compared to previous state-of-the-art results, and compared to running our system on the original dataset.


\setlength{\tabcolsep}{3pt}
\begin{table}[h]
\small
\centering
\caption{\label{tab:best_results}Our best classification accuracies for each testing set, with historical state-of-the-art accuracies and change in error rate for comparison.}

\begin{tabular}{lrrr}
  \hline
{\bf Dataset} & {\bf Historical} & {\bf Current} & {\bf $\Delta$ error}  \\
\hline
{\it Tratz}            &&&\\% 79.4\% & 90.3\% & -52.9\% \\
{\it \oshay Coarse}    &&&\\% 65.4\% & 86.2\% & -23.0\% \\
{\it \oshay Directed}  &&&\\% 65.1\% & 87.2\% & -23.1\% \\
{\it \oshay Fine}      &&&\\% 53.9\% & 85.1\% & -17.3\% \\
{\it Kim \& Baldwin}   &&&\\% 53.3\% & 55.1\% & -0.04\% \\
{\it Wordrobe}         &&&\\% N/A    & 82.3\% & N/A \\
\hline
\end{tabular}
\end{table}

The best condition (XXX) and the best augmentation dataset (PPDB L) are used for the test accuracies reported here. Table~\ref{tab:best_results} contains test set accuracies in an overview of previous state-of-the-art results next to the improved results from this work.

\section{Discussion}

\subsection{Dataset Augmentation}
In this paper, we compared the effects of using PPDB 2.0 as opposed to WordNet 3.0 for dataset augmentation.
For most cases, using PPDB 2.0 yielded better results.
The manually created WordNet and the automatically generated PPDB are two very different lexical resources made for different purposes.
It is nonetheless noteworthy that using an automatically generated resource by far outperforms a manually created and thoroughly checked one.
The results presented in this paper thus further support the quality of PPDB and its usefulness.\todo{This section is very important to the paper, and definitely needs more work.}

The differing performance between the two resourcescan be explained by the fact that significantly increasing the dataset size in the case of dataset augmentation is crucial.
This has been found in other fields such as computer vision etc., so why should this not be the case in NLP as well.
Furthermore, when augmenting datasets it is important to alter invariant properties of the data (see Section~\ref{sec:dataset_augmentation_background}).
Using only lemma forms from the same synset in WordNet should certainly be a very safe option
Using paraphrases, however, may seem less robust, as many paraphrases can have quite different meanings (e.g. \textit{miles} paraphrased as \textit{kilometers} (see Table~\ref{augment_examples})).
However, in the case of noun-compound classification, the invariance frame is apparently larger than that of a synonym.
It would be interesting to perform experiments with WordNet looking at whether including lemmas from relations of a given synset (e.g. \textit{cat}) such as hypernyms (e.g. \textit{feline}), hyponyms (e.g. \textit{siamese}) or co-hyponyms (e.g. \textit{dog}) would further aid performance.
The case of defining co-hyponyms would, however, be a challenge in itself, considering that these are not explicitly defined in WordNet and require constraints to be set in terms of how far removed the shared hypernym of two would-be co-hyponyms should be.
Such challenges further highlight the advantage of using PPDB for dataset augmentation, as such concerns are more simply covered by using different sizes of the PPDB.

\subsection{Unigram, Bigram and combination settings}

Differences.

\subsection{Embeddings}
Although the embeddings were not tuned to the task at hand, very promising results were obtained.
We expect that using embeddings which have been tuned to each dataset used will improve results further.

\subsection{Tratz dataset}
Far better than previous state of the art \citep{DimaHinrichs:2015,TratzHovy:2010}.

\subsection{\oshay dataset}
\citet{OseaghdhaCopestake:2013} use fewer labels in their study, as they exclude labels occuring 10 times or fewer.
Using dataset augmentation this problem is alleviated, since these labels occur more frequently, allowing the neural network to predict it more successfully.
Taking into account that a reduced tagset is used by the previous state-of-the-art study, the results obtained in this work are put in an even brighter light.

\subsection{Kim \& Baldwin dataset}
Results on the Kim \& Baldwin dataset proved comparably disappointing.
Although accuracy on most datasets increased in the range of 10\% to 30\%, only a few percent increase in accuracy was observed for this dataset.
This can be explained by the fact that performance is already close to human performance even when using the original data set.

Other reasons?

\subsection{Wordrobe dataset}
The results presented for the Wordrobe dataset are roughly similar to those obtained for the others.
This also constitutes the first results for noun compound interpretation of this dataset in the litterature.

\subsection{Generality}
How general is this dataset augmentation method?
Can it be extended to other tasks?

\subsection{Improvement beyond the state-of-the-art}

The procedure outlined in this paper resulted in improved performance as compared to a baseline system on all datasets, and state-of-the-art performance on some datasets.
Tuning various aspects of the learning architecture and using more sophisticated features would increase the classification performance further, likely outperforming the current state-of-the-art.
Training task-specific word embeddings and adding in linguistically motivated features, as done by e.g. \citet{OseaghdhaCopestake:2013}, would be a suitable first step in this direction.


\subsection{A look back at the related work section}
\todo[inline]{Talk about invariance, as in section 2}

\vspace{1cm}

\todo[inline]{Talk about robustness, as in section 2}

\section{Conclusions and Future Work}
We have shown that dataset augmentation can be applied to noun compound classification with substantial performance gains, resulting in state-of-the-art accuracy for 4 datasets.
Given the evident advantages of this method, future work should investigate the possibilities of applying this to other tasks and to other languages.


==> comp_sem/dataset_augmentation_text.tex <==

\begin{abstract}
  \absprelude The simplest way of increasing the generalisation ability of a machine learning model is to provide it with more training data.
  However, the availability of tagged training data is often limited, and creating more human annotated data is expensive.
  In this chapter we show how automatic linguistic dataset augmentation can be applied to semantic classification, thus increasing dataset sizes and system performance quickly and cheaply.
  We evaluate and compare the two lexical resources PPDB and WordNet, and apply our method to four annotated noun compound datasets and one dataset with animacy annotation.
  We use a simple feed-forward neural network architecture with features from off-the-shelf word embeddings, enriched with semantic relations from PPDB 2.0.
  The classification accuracy increases in the cross-validation setting for all noun compound datasets, and significant gains, as well as state-of-the art performance, are observed in the test set for one dataset.
%Previous systems which use complex features and learning architectures are outperformed using a simple neural network architecture with off-the-shelf word embedding features, coupled with augmented datasets.
  More complex features and task-specific embeddings are expected to further improve upon the gains obtained from our method.
\end{abstract}


\section{Introduction}

A general approach for artificially increasing the size of Natural Language Processing (NLP) datasets could lead to performance increases for a large number of NLP tasks, at little-to-no cost.
This is because the most straightforward manner of increasing the generalisation ability of a machine learning model is to provide it with more training data.
In practice, the amount of data available is often quite small, and creating more human annotated data is both time-consuming and expensive.
A relatively cheap way of getting more training data is to slightly alter the original training data and adding this to the dataset.
This technique is called \textit{dataset augmentation}.
%Although this is relatively simple in many machine learning applications, it is much more challenging in NLP.
%The advantage of having a general dataset augmentation method for Natural Language Processing (NLP) is that one could increase training set sizes, and thus performance for a large number of NLP tasks.

For some tasks, dataset augmentation is reasonably simple.
For instance, within computer vision, dataset augmentation is frequently done by scaling and rotating input images.
Since a given image can be scaled and rotated in many imaginable ways, datasets can be made much larger with relatively little effort.
One must take care not to apply transformations that are important to the problem at hand.
For example, optical character recognition (OCR) requires there to be a difference between the characters \textit{b, p, d} and \textit{q}, so horizontal flips and $180^{\circ}$ rotations are not suitable manners of augmenting such data \citep{BengioBook}.
Applying geometric transformations to atomic units such as words does not seem quite as straightforward as in the case of OCR, however.
Ideally one would want to generate new augmented training examples which are similar to the original training data, while maintaining as much information as possible, so that the label of the original training example is also applicable to the augmented training example.
We consider creating and evaluating a general dataset augmentation for NLP to be extremely challenging, and focus on a sub-discipline of NLP.
The aim of this chapter is thus to provide insight into how dataset augmentation can be done in the setting of semantic classification.
We approach this question using the tasks of noun compound interpretation and animacy classification as case studies.

% We investigate which of two lexical resources, one manually created and one automatically generated, is the most suited for dataset augmentation.
% We report on experiments on four annotated noun compound datasets \citep{Tratz:2011,Oseaghdha:2008,KimBaldwin:2005,Bos:2015} using the Paraphrase Database \citep{ppdb} and WordNet \citep{Miller:1995} for dataset augmentation by replacing constituents in each compound with (near-) synonyms.
% We use a simple neural network learning architecture with features from off-the-shelf word embeddings so as to highlight the advantage of applying dataset augmentation and facilitate replication of our work.

The rest of this chapter is structured as follows:
In Secton 2.2, related work on dataset augmentation, noun compound interpretation and animacy classification is presented.
Secton 2.3 contains an outline of the datasets used in this work.
The method is described in Secton 2.4.
In Secton 2.5 we present our results.
Secton 2.6 contains a discussion, and we conclude in Secton 2.7.

\section{Related work}

\subsection{Dataset Augmentation}
\label{sec:dataset_augmentation_background}

For many machine learning methods, and particularly for deep learning, appropriate dataset augmentation techniques are important to increase the generalisation ability of the model at hand.
Such techniques work well when invariant properties which the model should possess are manipulated.
For instance, in image recognition, a model should have invariance towards changes such as scaling and rotation (see e.g. \citet{Duin:1997,Tompson:2014}).
In speech recognition, data is often augmented by adding training examples with artificial background noise, or with the speed or tone of the speech signal altered \citep{Hannun:2014}.
The advantages of dataset augmentation lie not only in the increased dataset sizes, but also in the fact that adding such noisy input can increase the robustness of the model learned by a neural network.
This is due to the fact that the neural network is forced to learn a representation which is invariant to this added noise, which is especially relevant in the case of (deep) neural networks, as they are not particularly robust \citep{TangEliasmith:2010}.

In NLP, however, dataset augmentation is more intricate than in the aforementioned applications, as simple signal manipulation methods are not feasible.
One option is to increase training data sizes by manually rephrasing sentences.
\citet{DeVault:2011} show that expanding training data in this manner does improve results for dialogue systems.
However, as this is both expensive and time-consuming, an automatic method of augmenting natural language data is needed.
\citet{Gardent:2013} build upon this by automatically generating paraphrases using a pivoting translation approach with Google Translate, resulting in increased performance in a QA system.
Their approach has the drawback that it is relatively complex, and that reproducing their work would be challenging as the ever-changing online blackbox of Google Translate is used.
\citet{Zhang:2015} present experiments on text understanding, in which they make attempts at manipulating a dataset using a thesaurus obtained indirectly from WordNet \citep{Fellbaum:2005} via the LibreOffice project.
Words deemed by the authors as replaceable are extracted from a given text, and a random subset of these are replaced with a synonym.
This approach has several weaknesses, such as the fact that it is not clear what semantic relations exist between replaceable words and their candidates in the thesaurus.
Additionally, the use of such an opaque resource makes it difficult to systematically investigate what factors might influence the effect of dataset augmentation.
Finally, the authors note that with their already large dataset sizes, dataset augmentation does not have much impact.
A small increase in testing accuracy is obtained using their dataset augmentation method (98.3\% accuracy without augmentation, 98.4\% accuracy with augmentation).

Research on dataset augmentation for NLP consists of a very small body of work, and we argue that it is in need of more attention.
We contribute to previous work on dataset augmentation for NLP in three ways:
i) we outline a method of applying dataset augmentation;
ii) we compare two widely used lexical resources for this approach;
iii) we show that gains in classification accuracy can be achieved using a simple dataset augmentation procedure, and thus highlight the need of more research in this area.

\subsection{Noun Compound Interpretation}

Noun compounds (expressions consisting of a sequence of two or more nouns) are common in English.
The relation that is expressed between two nouns in a compound is not expressed explicitly, and it is a challenging task to classify this automatically.
For instance: the relation in 'leaf blower' is \mbox{\textsc{objective}}, whereas the relation in 'leaf temperature' is \mbox{\textsc{property}}.
Determining the relationships between such compounds is an important problem for a wide variety of NLP applications, such as machine translation \citep{baldwin:2004} and question answering \citep{ahn:2005}.
It is a difficult problem for various reasons (cf. \citet{jones:1983}), such as the fact that no proposed annotation scheme has been generally accepted.
The task has long been the subject of various research efforts, both in terms of developing resources and annotation schemes, as well as focussing on improving system performances on such datasets.

One of the earliest approaches is presented by \citet{Lauer:1995}, who uses corpus statistics to analyse compound nouns.
\citet{RosarioHearst:2001} attempt domain-specific noun compound relation classification, using medical texts.
\citet{KimBaldwin:2005} present a dataset with classification experiments based on calculating similarities between instances in the training and test set.
\citet{Girju:2005} use WordNet-based models and SVMs to classify noun compounds consisting of two and three words.
\citet{Oseaghdha:2008} constructs a dataset, and \citet{OseaghdhaCopestake:2013} report the current state-of-the-art experiments on this dataset.
\citet{TratzHovy:2010} present a dataset and experiments, and \citet{Tratz:2011} refines this dataset.
\citet{DimaHinrichs:2015} report the current state-of-the-art experiments on the Tratz dataset using features based on word embeddings \citep{Tratz:2011}.
\citet{Bos:2015} shows an analysis of a newly created dataset annotated via crowdsourcing.
As for languages other than English, \citet{Verhoeven:2012} report on experiments for Dutch and Afrikaans.

Our contributions to previous work on noun compound interpretation can be summed up as follows:
i) we improve upon previous classification results for two datasets;
ii) we show that word embeddings can be successfully applied to several such datasets, and show that architectural choices can markedly improve results;
iii) we show the benefits of applying dataset augmentation to this task.

\subsection{Animacy Classification}
Animacy is the semantic property of nouns denoting whether, or to what extent, the referent of that noun is alive, human-like or even cognitively sophisticated.
Several ways of characterising the animacy of such referents have been proposed in the literature, the most basic distinction being between animate and inanimate entities.
In such a binary scheme, examples of animate nouns might include \textit{author} and \textit{dog}, while examples of inanimate nouns might include \textit{table} and \textit{rock}.
More elaborate schemes tend to represent a hierarchy or continuum typically ranging from \textsc{human} $\rightarrow$ \textsc{non-human} $\rightarrow$ \textsc{inanimate} (cf. \citet{Comrie:1989}), potentially with other categories in between these.
In various languages, animacy affects linguistic phenomena such as case marking and argument realisation.
Furthermore, hierarchical restrictions are often imposed by animacy, e.g., with subjects tending to be higher in an animacy hierarchy than objects \citep{DahlFraurud:1996}.
Even though animacy is rarely overtly marked in English, it still influences the choice of certain grammatical structures, such as the choice of relative pronouns (e.g. who vs. which).

Although seemingly overlooked in the past, animacy has in later years been shown to be an important feature for NLP.
\citet{OvrelidNivre:2007} found that the accuracy of a dependency parser for Swedish could be improved by incorporating a binary animacy distinction.
Other work has highlighted animacy as relevant for anaphora and coreference resolution \citep{OrasanEvans:2007,Lee:2013} and verb argument disambiguation \citep{DellOrletta:2005}.

Our contributions to previous work on animacy classification  can be summed up as follows:
i) we show that word embeddings can be successfully used for such datasets;
ii) we show the effects of applying dataset augmentation to this task.

\section{Datasets}
We experiment on four annotated noun compound datasets and one dataset with animacy annotation.
All of these datasets are in English.
The noun compound datasets contain two-noun compounds without any further context.
The animacy dataset contains noun phrases annotated with an animacy label.
The noun compound datasets differ in the vocabularies of relations which they encode.
An overview of the datasets is shown in Table~\ref{tab:datasets}.

\setlength{\tabcolsep}{5pt}
\begin{table}[h]
\centering
\caption{\label{tab:datasets}Overview of the datasets used in this chapter, with the number of annotated entities and tags in each dataset.}
\begin{tabular}{llrr}
\hline
{\bf Dataset} & {\bf Type}& {\bf Annotated entities} & {\bf Tags}  \\
\hline
{\bf Tratz}          & Noun Compounds & 19,158   & 37 \\
{\bf \oshay}         & Noun Compounds & 1,443    & 6 / 11 / 37\\
{\bf Kim \& Baldwin} & Noun Compounds & 2,169    & 20 \\
{\bf Wordrobe}       & Noun Compounds & 965      & 25 \\
{\bf Switchboard}    & Animacy        & 200,000  &  10 \\
\hline
\end{tabular}
\end{table}

\subsection{\citet{Tratz:2011} dataset}

The Tratz dataset \citep{Tratz:2011} is the largest annotated noun compound dataset which is publicly available, containing 19,158 compounds annotated with 37 semantic relations.\footnote{\citet{Tratz:2011} dataset:\\ \url{http://isi.edu/publications/licensed-sw/fanseparser/}}
The inventory of relations consists of semantic categories resembling those previously proposed by \citet{Barker:1998} and \citet{Girju:2005}.
The altered inventory of relations, as compared to \citet{Barker:1998}, is motivated by \citet{TratzHovy:2010} by the resulting increased inter-annotator agreement.
Furthermore, \citet{Tratz:2011} motivates the revision of relations by the necessity of creating a better mapping between prepositional paraphrases and noun compound relations.
The state-of-the-art results on this dataset are 77.12\% (accuracy on test) and 79.38\% (accuracy on development) \citep{DimaHinrichs:2015}.

\subsection{\citet{Oseaghdha:2008} dataset}

The \oshay dataset is a much smaller annotated noun compound dataset, containing 1,443 compounds annotated with semantic relations at three levels of granularity \citep{Oseaghdha:2008}.\footnote{\citet{Oseaghdha:2008} dataset: \url{http://www.cl.cam.ac.uk/~do242/Resources/}}
The annotated relations can be divided into three subsets:
\begin{itemize}
  \item Coarse: \textsc{be}, \textsc{have}, \textsc{in}, \textsc{actor}, \textsc{instrument}, \textsc{about} (6 labels);
  \item Directed: coarse relations with directionality (11 labels);
  \item Fine: fine-grained labels corresponding to annotation rules and which constituents fill which relation slots (37 labels).
\end{itemize}
The state-of-the-art results on this dataset are 65.4\% (Coarse), 65.1\% (Directed) and 53.9\% (Fine) \citep{OseaghdhaCopestake:2013}.


\subsection{\citet{KimBaldwin:2005} dataset}

The Kim \& Baldwin dataset is another small annotated noun compound dataset, containing 2,169 compounds annotated with 20 labels \citep{KimBaldwin:2005}.\footnote{\citet{KimBaldwin:2005} dataset: \url{http://multiword.sourceforge.net}}
This dataset notably has a low inter-annotator agreement, and relatively unevenly distributed data \citep{TratzHovy:2010}.
The state-of-the-art result on this dataset is 53.3\% \citep{KimBaldwin:2005}.

\subsection{Wordrobe dataset}
\citet{Bos:2015} describe a gamification-based method for obtaining noun compound annotations.
Wordrobe \citep{wordrobe} is used in order to tag noun compounds with relations based on 26 prepositions.
Overall, 25 of these are used by the annotators on a dataset containing 965 compounds.\footnote{Wordrobe dataset \citep{Bos:2015}: \url{http://gmb.let.rug.nl/data.php}}
To the best of our knowledge, there is no previous work reporting classification accuracies on this dataset.

\subsection{Switchboard Corpus}

The NXT Switchboard corpus represents (one of) the largest resources with animacy annotation \citep{calhoun:2010}.
This spoken language corpus contains high quality manual annotation of animacy for nearly 200,000 noun phrases \citep{zaenen:2004}.
Furthermore, the annotation is fairly fine-grained, as a total of ten animacy categories are used, with a few additional tags for mixed animacy and cases in which annotators were uncertain.
This scheme can be arranged hierarchically, so that the classes concrete, non-concrete, place and time are grouped as inanimate, while the remaining classes are grouped as animate.
Evaluating on the Switchboard corpus allows for direct comparison of results to \citet{bowman:2012} and \citet{bjerva:14:eacl}.

\subsection{Dataset preprocessing}
The Switchboard corpus consists of transcribed spoken data, and also contains disfluency markers in the transcribed texts.
As these markers likely have little-to-no bearing on the animacy of an entity, a preprocessing step consisted of removing all such disfluencies (labelled with the tag \textit{UH}).
We further strip each training instance in the Switchboard corpus down to contain the head noun of the annotated NP and at most one extra context word.
This is done in order to allow for the same dataset augmentation procedure to be carried out for this dataset as for the noun compound datasets.

We also apply a simple preprocessing step for all datasets, consisting of converting all words to lower case.
This is necessary since the embeddings we use are trained on lower-cased text, whereas several of the datasets contain words with upper case letters (e.g. proper nouns in the Tratz dataset).

\section{Method}

\setlength{\tabcolsep}{1.5pt}
\begin{table*}[t]
\tiny
\centering
\caption{\label{tab:augment_examples}Randomly chosen examples of augmented compounds with one replaced constituent using both WordNet conditions and all PPDB sizes, with the source compound and its annotated relation group in the Tratz dataset \citep{Tratz:2011}.}
\begin{tabular}{llllll}
  \hline
  {\bf Relation} & \textsc{complement} & \textsc{topic} & \textsc{objective} & \textsc{purpose} & \textsc{location} \\
  \hline
  \textsc{original} & family background & arms talk & gold dealer & care center & border clash \\
  \textsc{ppdb s} & families background & weapons talk & gold concessionaire & care centre & frontier clash \\
  \textsc{ppdb m} & family context & armaments talk & gold distributor & attention center & boundary clash \\
  \textsc{ppdb l} & household background & arm talk & kim dealer & caring center & boundaries clash \\
  \textsc{ppdb xl} & familia background & weaponry talk & dorado dealer & soins center & frontire clash \\
  \textsc{ppdb xxl} & range background & booby talk & air dealer & saves center & edges clash \\
  \textsc{ppdb xxxl} & genealogy background & utensils talk & thumb dealer & payload center & limitation clash \\
  \textsc{wn first} & menage background & munition talk & gold bargainer & tending center & border clangoring \\
  \textsc{wn all} & fellowship background & blazon talk & u dealer & forethought center & molding clash \\
\hline
\end{tabular}
\end{table*}

\setlength{\tabcolsep}{4pt}

\subsection{Lexical resources}
The dataset augmentation method outlined in this chapter requires lexical resources in order to be applied.
We experiment with using two such resources: The Paraphrase Database and WordNet.

\subsubsection*{The Paraphrase Database}
\noindent The Paraphrase Database (PPDB) is a collection of paraphrases which has been automatically constructed using bilingual pivoting \citep{ppdb}.
This resource includes paraphrases of lexical units as well as longer phrases, and exists in six sizes following a continuum from highest precision and lowest recall, to lowest precision and highest recall (S, M, L, XL, XXL, XXXL).
The smallest versions (S, M) contain a large proportion of equivalent paraphrases, whereas larger versions (L, XL) increasingly contain paraphrases which entail each other, and the largest versions (XXL, XXXL) contain a large amount of otherwise related or independent paraphrases \citep{PavlickBosEtAl:2015}.
The recently released PPDB 2.0 adds to the original PPDB by reranking paraphrases in a better way than the previous version as judged by humans, as well as including explicit entailment relations between paraphrases, style classification and distances obtained from a word embedding model \citep{ppdb2}.
The entailment relations used are: equivalence, forward and reverse entailment, opposites, independent, and other \citep{PavlickBosEtAl:2015}.

\subsubsection*{WordNet}
\noindent WordNet (WN) is a manually created lexical resource in which words are categorised into groups of synonyms called synsets \citep{Miller:1995,Fellbaum:2005}.
Synonyms of a given word can be looked up by, e.g., retrieving the most common sense of that word in WN and extracting all lemmas of that synset, or by extracting all lemmas of all senses of a word.
We use WN version 3.0 in our experiments.

\subsection{Dataset Augmentation for Semantic Classification}
We use PPDB 2.0 as a source of synonyms and near-synonyms.\footnote{PPDB 2.0: \url{http://paraphrase.org}}
Since we are experimenting with datasets consisting of noun compounds, we use a subset of the PPDB filtered to contain only nominal paraphrases.
This is done based on the constituent tag available for each paraphrase in the PPDB.
Experiments are run using all sizes of the PPDB, yielding six settings (\textsc{ppdb s}, \textsc{ppdb m}, $\ldots$, \textsc{ppdb xxxl}).

We also experiment using WordNet 3.0 as a source of synonyms and near-synonyms.
We extract these in two ways.
In the \textsc{wn first} setting, we use all lemmas of the most frequent sense of the given word.
In the \textsc{wn all} setting, we use all lemmas of \textit{all} senses of the given word.

Our dataset augmentation procedure is as follows.
Every training instance (e.g. \textit{dog house}) in the training sets is split into its two constituents (e.g. \textit{dog} and \textit{house}).
We generate new augmented training instances in three ways.
In one condition, \textsc{unigram}, we keep one constituent constant (e.g. \textit{dog}), while replacing the other (e.g. \textit{house}) with available synonyms and near-synonyms (e.g. \textit{home}, \textit{chamber}).
We generate augmented examples in which the first constituent is changed as well as examples where the second constituent is changed.
In the case of the PPDB, all paraphrases in the given setting are taken to be synonyms and near-synonyms.
In the case of WordNet, all lemmas of the synset(s) at hand are used.
In the second condition, \textsc{bigram}, we replace both constituents of the compound with a bigram synonym or near-synonym.
We also combine these two approaches in the third condition, \textsc{unigram+bigram}.
This results in a total of three conditions and nine settings (six PPDB settings, two WN settings and one unaugmented/original setting).

We also experimented with a variation of the \textsc{unigram} condition on the noun compound datasets.
In this variation, we made two new conditions -- one in which only the first word of the compound was replaced, and one in which only the second word was replaced.
However, no differences were found between these two conditions, and lower accuracies were obtained than in the standard \textsc{unigram} condition.

The result of this procedure is a much larger list of training instances (e.g. \textit{dog home}, \textit{canine house}, \textit{hound home}).
Note that the training instances are kept in the training set.
Although the augmented training instances, such as listed above, represent somewhat awkward or non-natural phrasings of the compound \textit{dog house}, they are assumed to convey the same relation as the original compound.
That is to say, both \textit{dog house} and \textit{canine house} should be labelled \textsc{user-recipient} if following the annotation scheme in \citet{Tratz:2011}.
Randomly chosen examples of augmented compounds with one replaced constituent are shown in Table~\ref{tab:augment_examples} with the original compound and its relation group in the Tratz dataset.
Depending on the dataset and source of \mbox{(near-)synonyms}, the new training sets are scaled from as little as 1.2 times (PPDB S) to as much as three orders of magnitude (PPDB XXXL) of the original size.
The smallest augmented datasets thus contain a minority of augmented examples, whereas original examples are outnumbered in the largest augmented datasets.
Figure~\ref{fig:dataaug_sizes} contains an overview of augmented sizes.


\begin{figure*}[t!]
  \centering
  %\includegraphics[width=\textwidth,trim=0 3mm 0 7mm,clip]{legend_wide}
  \begin{subfigure}{0.48\textwidth}
  \includegraphics[width=\textwidth,trim=0 0 0 15mm,clip]{dataaug_sizes_ppdb}
  \caption{\label{fig:dataaug_sizes_ppdb}PPDB settings}
  \end{subfigure}
  \begin{subfigure}{0.48\textwidth}
  \includegraphics[width=\textwidth,trim=0 0 0 15mm,clip]{dataaug_sizes_wn}
  \caption{\label{fig:dataaug_sizes_wn}WN settings}
  \end{subfigure}
  \caption{\label{fig:dataaug_sizes}Training set size changes for all datasets under all settings in the \textsc{unigram+bigram} condition. The y-axis depicts the size increase coefficient on a log scale. The x-axis depicts dataset augmentation sizes.}
\end{figure*}

%We considered controlling the augmentation process by asserting that we do not include augmented noun compounds identical to ones in the development sets.
%The experiments reported in this chapter do not make this assertion, as this might increase the discrepancy between the development set and test set conditions.

\subsection{Features}
We use two types of features in our experiments: pre-trained word embeddings, and entailment relations obtained from PPDB 2.0.

\subsubsection*{Word embeddings}
\noindent Continuous space representations of words are currently the backbone of several high-performing approaches in NLP.
The distributional hypothesis, summarised as: `You shall know a word by the company it keeps' \citep{firth} is the basis for many approaches of obtaining such representations.
Word embeddings are an example of such a model (e.g. \citet{collobert:2008}), and have been found to encapsulate interesting semantic properties; in a model presented by \citet{Mikolov:13:Regularities}, the result when calculating
\mbox{$\overrightarrow{\textsc{king}} - \overrightarrow{\textsc{man}}
+ \overrightarrow{\textsc{woman}}$},
is close to $\overrightarrow{\textsc{queen}}$.
Although the seemingly magical properties of the Mikolov embeddings have been disspelled (cf. \citet{Levy:2015}), they perform remarkably well.

In this work we use publicly available embeddings, with 300 dimensions, which have been pre-trained on about 100 billion words.\footnote{Pre-trained embeddings: \url{http://code.google.com/p/word2vec/}}
This choice was made so as to facilitate reproducibility of our work.
However, previous work has highlighted the importance of parameter selection in word embeddings (cf. \citet{Tang:2014,Levy:2015}), and we therefore expect there to be further room for improvement to the scores reported in this chapter when using embeddings tuned to the task at hand.

\subsubsection*{Linguistic information}
\noindent We experiment with using the entailment relations obtained from PPDB 2.0 as an extra feature in the experiments which employ this resource.
For each augmented training example, a feature vector with one-hot encoding is concatenated to the standard feature vector.
Original examples in the training, development and test sets contain zeroes in each of these extra feature dimensions.

\subsection{Experimental setting}
We use a simple feed-forward neural network in our classification experiments, implemented in Keras using Theano \citep{theano:orig,theano:nips}.\footnote{Keras: \url{http://keras.io/}}
The architecture used is illustrated in Figure~\ref{fig:nn}.
We use a single hidden layer, with the same amount of neurons as the input layer ($n=600$, except when using the entailment relation features, where $n=604$).
We use the ADAM optimisation algorithm, which adapts the learning rate for different layers instead of requiring tuning as in SGD \citep{Kingma:2014}.
The loss function used is categorical cross entropy.
We use a batch size of 50 and train over the course of 500 epochs.
Initialisation is done using the method outlined by \citet{lecun:1998}, in which initial weights are drawn from a uniform distribution scaled by the square root of the number of inputs.
We use maxout, which effectively learns the most appropriate activation function of each neuron \citep{maxout}.
Maxout can be advantageous compared to the currently popular Rectified Linear Units (ReLUs), since ReLUs can get stuck by learning to de-activate and never again be re-activated \citep{rectifier,maxout}.
The output layer uses a softmax activation function.
We employ dropout as regularisation \citep{dropout}. This essentially entails randomly nullifying a certain proportion of neuron activations in each forward pass, which encourages neurons not to be dependent on the values of other neurons (since they can and do disappear at any time), thus increasing the robustness and generalisation ability of the neural network.
All hyper-parameters except for dropout probabilities are kept constant in all conditions, settings, and for all datasets.
We vary dropout probabilities in the range $[p=0.1,p=0.5]$ for the input layer and $[p=0.3,p=0.8]$ for the hidden layer.
Lower dropout probabilities for the input layer were chosen since this is shown to be beneficial in \citet{dropout}.
The dropout probabilities yielding the best cross-validation performance are used in all reported results.

We also experimented using other architectural choices, varying the amount of layers, activation functions, optimisation algorithms and initialisations.
The final architectural choices reflect the ones consistently yielding the best accuracies on the development sets.

\begin{figure}[h]
  \centering
  \resizebox{11cm}{4.5cm}{
    \input{comp_sem/neural_network}
  }
  \caption{\label{fig:nn}Neural network architecture used in our experiments. Each layer has $n=600$ units, except for the output layer with $n=k$ units whrere $k$ is the amount of semantic relations to classify for the given dataset. The inputs are given by mapping both nouns in each given compound to their vectors in the word embeddings used, and concatenating these.}
\end{figure}

\subsection{Evaluation}
For the Kim \& Baldwin dataset we use the official training / testing splits, and use 10\% of the training data as development data.
For all other datasets, the data is randomly shuffled and split into 20\% / 10\% / 70\% for testing, development, and training, respectively.
We use the combined training and development splits to construct 5-fold cross-validation sets.
Test sets were held-out until final evaluation took place.

For evaluation on the test sets, the overall best combination of conditions (PPDB vs. WordNet, and \textsc{unigram} vs. \textsc{bigram} vs. \textsc{unigram+bigram}) is chosen based on the cross-validation results.
After one pass over only the training set, the development data is added to the training set and training runs until the previously best performing epoch, following \citet{BengioBook}.
The resulting test set accuracy is then reported.

Statistical significance tests on the test sets are performed using Wilcoxon's test \citep{harnett:1982}, which is a non-parametric test suitable for simple NLP metrics such as accuracy \citep{yeh:2000}.
In NLP, p-values are particularly fickle and are susceptible to, e.g., sample sizes and the choice of metrics \citep{Sogaard:2014}.
We therefore follow the authors' recommendation of using a significance cutoff of $p<0.0025$ in order to arrive at the probability of a false research finding at less than $5\%$.

\section{Results}

A statistically significant improvement ($p<0.0025$) is found when comparing test set performance in an unaugmented vs. augmented setting on the Tratz dataset (see Table~\ref{tab:best_results}).
For the Tratz dataset state-of-the-art performances are also achieved (compared to \citet{DimaHinrichs:2015}).
No significant difference is found for the other datasets at our chosen alpha-level ($0.01 > p \geq 0.0025$).

\setlength{\tabcolsep}{4pt}
\begin{table}[h!]
\small
\centering
\caption{\label{tab:best_results}Test set accuracies under unaugmented and augmented conditions. The augmented conditions use the best performing parameters per dataset as judged in the cross-validation setting. Significant differences between the unaugmented and augmented setting at $p<0.0025$ are suffixed with an asterisk ($*$). A suffixed $\bullet$ indicates $0.01 > p \geq 0.0025$. A prefixed star ($\star$) indicates improvement on the state-of-the-art results found in the literature.}
  \begin{tabular}{lrr}
    \hline
  {\bf Dataset} & {\bf Unaugmented} & {\bf Augmented} \\
  \hline
  {\bf Tratz}             & $78.52\%$ & $\star\textbf{78.88\%*}$ \\
  {\bf \oshay Coarse}     & $58.13\%$ & $\textbf{59.86\%}\bullet$  \\
  {\bf \oshay Directed}   & $54.67\%$ & $\textbf{55.02\%}\bullet$  \\
  {\bf \oshay Fine}       & $47.41\%$ & $\textbf{48.44\%}\bullet$  \\
  {\bf Kim \& Baldwin}    & $50.66\%$ & $\textbf{51.32\%}\bullet$ \\
  {\bf Wordrobe}          & $44.79\%$ & $\textbf{58.38\%}\bullet$  \\
  {\bf Switchboard}       & $84.55\%$ & $\textbf{84.56\%\ \ }$  \\
  \hline
  \end{tabular}
\end{table}

Table~\ref{tab:dev_results} shows the effect of the WN and PPDB settings used for dataset augmentation on classification accuracy using 5-fold cross validation on all datasets.
Table~\ref{tab:unigram_dev_results} contains cross-validation accuracies under the \textsc{unigram} condition, Table~\ref{tab:bigram_dev_results} under the \textsc{bigram} condition, and Table~\ref{tab:both_dev_results} under the \textsc{unigram+bigram} condition.
The \textsc{unigram} and \textsc{unigram+bigram} conditions yield better results in all cases.
Within these conditions, the \textsc{ppdb s} setting yields the best results in most cases, with larger sizes yielding lower results.
Exceptions to this are the \oshay fine dataset, where \textsc{ppdb l} performs the best, and the Kim \& Baldwin dataset, where \textsc{ppdb xl} performs the best.
Dataset augmentation improves upon an unaugmented baseline on all datasets in the cross-validation setting.

Table~\ref{tab:entailment_results} contains a comparison of results in the cross-validation setting when including and excluding entailment relation features from the PPDB.
Including this feature increases classification accuracy for all datasets and in all settings, except for a few minor exceptions.

\setlength{\tabcolsep}{2pt}
\begin{table*}[p!]
\tiny
\centering
\caption{\label{tab:dev_results}Mean cross-validation accuracies for all datasets under the \textsc{unigram}, \textsc{bigram}, and \textsc{unigram+bigram} conditions. PPDB conditions include entailment relation features. Brackets contain the standard deviations as calculated across five folds. Bold numbers indicate the best accuracies within a condition. Asterisks indicate the best accuracies across conditions.}
  \begin{subtable}{\textwidth}
    \caption{\label{tab:unigram_dev_results}\textsc{unigram} condition}
    \begin{tabular}{lrrrrrr}
      \hline
      {\bf Setting} & {\bf Tratz} & {\bf \oshay Coarse} & {\bf \oshay Dir.} & {\bf \oshay Fine} & {\bf Kim\&Baldwin}  & {\bf Wordrobe} \\
      \hline
      \textsc{original} & $79.4$ $(0.0)$ & $62.3$ $(0.9)$ & $58.8$ $(1.1)$ & $50.9$ $(0.6)$ & $52.5$ $(0.4)$ & $54.2$ $(3.0)$ \\
      \textsc{ppdb s} & $\textbf{79.6}$ $(0.1)$ & $\textbf{*64.0}$ $(1.2)$ & $58.8$ $(0.8)$ & $51.2$ $(0.8)$ & $53.2$ $(0.6)$ & $\textbf{*54.7}$ $(1.5)$ \\
      \textsc{ppdb m} & $79.6$ $(0.1)$ & $62.3$ $(0.6)$ & $58.1$ $(0.5)$ & $50.9$ $(0.6)$ & $52.9$ $(0.4)$ & $53.1$ $(0.9)$ \\
      \textsc{ppdb l} & $79.3$ $(0.2)$ & $63.3$ $(0.9)$ & $58.8$ $(0.5)$ & $\textbf{*52.2}$ $(0.9)$ & $53.3$ $(0.3)$ & $53.6$ $(1.1)$ \\
      \textsc{ppdb xl} & $78.0$ $(0.1)$ & $62.6$ $(1.3)$ & $56.1$ $(0.3)$ & $48.8$ $(0.6)$ & $\textbf{53.4}$ $(0.4)$ & $47.9$ $(0.9)$ \\
      \textsc{ppdb xxl} & $77.5$ $(0.1)$ & $62.1$ $(0.8)$ & $55.3$ $(0.4)$ & $47.1$ $(0.7)$ & $53.1$ $(0.4)$ & $45.1$ $(1.0)$ \\
      \textsc{ppdb xxxl} & $77.3$ $(0.1)$ & $61.8$ $(0.8)$ & $51.0$ $(0.3)$ & $45.0$ $(0.5)$ & $52.7$ $(0.3)$ & $44.3$ $(1.1)$ \\
      \textsc{wn first} & $78.1$ $(0.1)$ & $61.9$ $(0.9)$ & $57.1$ $(0.7)$ & $48.8$ $(0.9)$ & $51.9$ $(0.2)$ & $52.1$ $(0.7)$ \\
      \textsc{wn all} & $74.5$ $(0.0)$ & $60.6$ $(0.5)$ & $53.3$ $(0.6)$ & $44.3$ $(0.6)$ & $52.5$ $(0.3)$ & $47.9$ $(0.3)$ \\
    \hline
    \end{tabular}
  \end{subtable}

  \vspace{5mm}

  \begin{subtable}{\textwidth}
    \caption{\label{tab:bigram_dev_results}\textsc{bigram} condition}
    \begin{tabular}{lrrrrrr}
      \hline
      {\bf Setting} & {\bf Tratz} & {\bf \oshay Coarse} & {\bf \oshay Dir.} & {\bf \oshay Fine} & {\bf Kim\&Baldwin}  & {\bf Wordrobe}\\
      \hline
      \textsc{original}  & $79.4$ $(0.0)$ & $62.3$ $(0.9)$ & $58.8$ $(1.1)$ & $50.9$ $(0.6)$ & $52.5$ $(0.4)$ & $\textbf{54.2}$ $(3.0)$ \\
      \textsc{ppdb s}  & $\textbf{79.7}$ $(0.1)$ & $\textbf{63.5}$ $(1.1)$ & $\textbf{59.2}$ $(0.9)$ & $\textbf{51.4}$ $(0.7)$ & $52.2$ $(0.3)$ & $53.1$ $(1.9)$ \\
      \textsc{ppdb m}  & $79.6$ $(0.1)$ & $62.5$ $(0.7)$ & $58.3$ $(0.6)$ & $50.3$ $(0.7)$ & $52.1$ $(0.5)$ & $51.4$ $(2.0)$ \\
      \textsc{ppdb l}  & $79.4$ $(0.2)$ & $61.5$ $(1.0)$ & $58.4$ $(0.5)$ & $50.9$ $(0.5)$ & $53.5$ $(0.4)$ & $53.0$ $(1.2)$ \\
      \textsc{ppdb xl} & $78.2$ $(0.2)$ & $61.4$ $(1.1)$ & $58.0$ $(0.4)$ & $49.9$ $(0.9)$ & $\textbf{54.2}$ $(0.5)$ & $47.2$ $(0.9)$ \\
      \textsc{ppdb xxl} & $77.6$ $(0.1)$ & $61.2$ $(1.0)$ & $54.0$ $(0.2)$ & $47.0$ $(0.8)$ & $54.1$ $(0.3)$ & $42.3$ $(1.0)$ \\
      \textsc{ppdb xxxl} & $77.3$ $(0.1)$ & $60.1$ $(0.7)$ & $51.2$ $(0.4)$ & $44.2$ $(0.5)$ & $53.9$ $(0.4)$ & $41.0$ $(1.1)$ \\
      \textsc{wn first} & $77.5$ $(0.1)$ & $61.2$ $(0.4)$ & $56.4$ $(1.1)$ & $50.2$ $(0.9)$ & $53.4$ $(0.5)$ & $54.2$ $(2.0)$ \\
      \textsc{wn all} & $67.6$ $(0.2)$ & $54.7$ $(0.9)$ & $50.9$ $(1.0)$ & $40.5$ $(0.4)$ & $51.0$ $(0.5)$ & $50.5$ $(0.9)$ \\
    \hline
    \end{tabular}
  \end{subtable}

  \vspace{5mm}

  \begin{subtable}{\textwidth}
    \caption{\label{tab:both_dev_results}\textsc{unigram+bigram} condition}
    \begin{tabular}{lrrrrrr}
      \hline
      {\bf Setting} & {\bf Tratz} & {\bf \oshay Coarse} & {\bf \oshay Dir.} & {\bf \oshay Fine} & {\bf Kim\&Baldwin}  & {\bf Wordrobe}\\
      \hline
      \textsc{original} & $79.4$ $(0.0)$ & $62.3$ $(0.9)$ & $58.8$ $(1.1)$ & $50.9$ $(0.6)$ & $52.5$ $(0.4)$ & $\textbf{54.2}$ $(3.0)$ \\
      \textsc{ppdb s} & $\textbf{*80.0}$ $(0.1)$ & $\textbf{63.7}$ $(0.9)$ & $\textbf{*59.5}$ $(1.0)$ & $\textbf{51.6}$ $(1.1)$ & $52.3$ $(0.2)$ & $53.6$ $(1.1)$ \\
      \textsc{ppdb m} & $79.6$ $(0.1)$ & $62.6$ $(0.8)$ & $58.1$ $(0.8)$ & $50.5$ $(1.1)$ & $52.8$ $(0.5)$ & $52.1$ $(1.1)$ \\
      \textsc{ppdb l} & $79.4$ $(0.1)$ & $61.9$ $(0.9)$ & $58.5$ $(1.3)$ & $50.2$ $(0.5)$ & $52.9$ $(0.4)$ & $53.6$ $(1.2)$ \\
      \textsc{ppdb xl} & $78.1$ $(0.2)$ & $61.6$ $(0.6)$ & $57.4$ $(1.0)$ & $49.1$ $(0.7)$ & $\textbf{*54.7}$ $(0.8)$ & $48.4$ $(0.6)$ \\
      \textsc{ppdb xxl} & $77.6$ $(0.1)$ & $61.6$ $(0.7)$ & $55.0$ $(1.1)$ & $48.5$ $(0.4)$ & $54.4$ $(0.4)$ & $41.3$ $(0.9)$ \\
      \textsc{ppdb xxxl} & $77.2$ $(0.1)$ & $60.0$ $(0.8)$ & $53.2$ $(0.9)$ & $44.1$ $(0.5)$ & $54.0$ $(0.3)$ & $40.1$ $(1.2)$ \\
      \textsc{wn first} & $77.5$ $(0.1)$ & $59.9$ $(0.4)$ & $55.7$ $(1.3)$ & $47.8$ $(0.9)$ & $51.2$ $(0.2)$ & $52.6$ $(1.0)$ \\
      \textsc{wn all} & $69.4$ $(0.2)$ & $55.0$ $(0.7)$ & $51.2$ $(0.7)$ & $38.8$ $(0.5)$ & $51.3$ $(0.2)$ & $49.0$ $(0.4)$ \\
    \hline
    \end{tabular}
  \end{subtable}

\vspace{5mm}

\setlength{\tabcolsep}{1.2pt}
\caption{\label{tab:entailment_results}Mean cross-validation accuracies for all datasets without the use of entailment relation features. Accuracies are averaged across the \textsc{unigram}, \textsc{bigram} and \textsc{unigram+bigram} conditions and five folds. Brackets contain the accuracy difference as compared to including the entailment relation features.}
\begin{tabular}{lrrrrrr}
  \hline
  {\bf Setting} & {\bf Tratz} & {\bf \oshay Coarse} & {\bf \oshay Dir.} & {\bf \oshay Fine} & {\bf Kim\&Baldwin}  & {\bf Wordrobe}\\
  \hline
  %\textsc{original} & $79.4$ $(0.0)$ & $62.3$ $(0.0)$ & $58.8$ $(0.0)$ & $50.9$ $(0.0)$ & $52.5$ $(0.0)$ & $54.2$ $(0.0)$ \\
  \textsc{ppdb s} & $79.4$ $(-0.3)$ & $62.4$ $(-1.3)$ & $57.3$ $(-1.9)$ & $49.8$ $(-1.6)$ & $52.4$ $(-0.2)$ & $52.5$ $(-1.7)$ \\
  \textsc{ppdb m} & $79.2$ $(-0.4)$ & $61.6$ $(-0.9)$ & $57.7$ $(-0.7)$ & $50.2$ $(-0.4)$ & $52.6$ $(\pm0.0)$ & $52.0$ $(-1.8)$ \\
  \textsc{ppdb l} & $79.1$ $(-0.3)$ & $62.5$ $(-1.0)$ & $58.2$ $(-0.4)$ & $50.7$ $(-1.2)$ & $52.8$ $(-0.4)$ & $51.4$ $(-2.0)$ \\
  \textsc{ppdb xl} & $77.7$ $(+0.1)$ & $60.7$ $(-0.9)$ & $56.1$ $(-1.0)$ & $47.9$ $(-1.4)$ & $53.2$ $(-0.9)$ & $47.4$ $(-0.4)$ \\
  \textsc{ppdb xxl} & $77.4$ $(-0.2)$ & $60.6$ $(-1.0)$ & $54.6$ $(-0.2)$ & $47.1$ $(-0.4)$ & $53.0$ $(-0.9)$ & $41.4$ $(-1.5)$ \\
  \textsc{ppdb xxxl} & $77.1$ $(-0.2)$ & $59.7$ $(-0.9)$ & $54.7$ $(-0.7)$ & $44.0$ $(-0.4)$ & $53.5$ $(\pm0.0)$ & $40.3$ $(-1.5)$ \\
\hline
\end{tabular}
\end{table*}

Table~\ref{tab:animacy_results} contains cross-validation results for the animacy classification task.
Dataset augmentation does not yield improved performance under any condition.

\begin{table*}[t]
\setlength{\tabcolsep}{6pt}
\centering
\caption{\label{tab:animacy_results}Mean cross-validation accuracies for the Animacy classification task on the Switchboard dataset.}
\begin{tabular}{lrrr}
  \hline
  {\bf Setting} & {\bf Switchboard unigram} & {\bf Switchboard bigram} & {\bf Switchboard both}\\
  \hline
  \textsc{ppdb o}    & \textbf{$84.5$} $(0.1)$ & \textbf{$84.5$} $(0.1)$ & \textbf{$84.5$} $(0.1)$ \\
  \textsc{ppdb s}    & $84.4$ $(0.2)$ & $84.2$ $(0.1)$ & $84.4$ $(0.1)$ \\
  \textsc{ppdb m}    & $84.4$ $(0.1)$ & $84.3$ $(0.2)$ & $84.5$ $(0.3)$ \\
  \textsc{ppdb l}    & $84.5$ $(0.3)$ & $84.4$ $(0.1)$ & $84.5$ $(0.2)$ \\
  \textsc{ppdb xl}   & $84.3$ $(0.1)$ & $84.1$ $(0.3)$ & $84.1$ $(0.3)$ \\
  \textsc{ppdb xxl}  & $84.2$ $(0.1)$ & $84.0$ $(0.2)$ & $83.9$ $(0.2)$ \\
  \textsc{ppdb xxxl} & $84.1$ $(0.1)$ & $84.2$ $(0.1)$ & $83.7$ $(0.2)$ \\
  \textsc{wn first}  & $84.4$ $(0.1)$ & $84.3$ $(0.2)$ & $84.2$ $(0.1)$ \\
  \textsc{wn all}    & $84.2$ $(0.2)$ & $84.1$ $(0.1)$ & $84.1$ $(0.3)$ \\
\hline
\end{tabular}
\end{table*}

% \setlength{\tabcolsep}{2pt}
% \begin{table*}[t]
% \tiny
% \centering
% \caption{\label{tab:dev_results_spec}Mean cross-validation accuracies for all noun compound datasets under the \textsc{first} and \textsc{last} conditions. PPDB conditions include entailment relation features. Bold numbers indicate the best accuracies within a condition. Asterisks indicate the best accuracies across these conditions.}
%   \begin{subtable}{\textwidth}
%     \caption{\label{tab:first_dev_results}\textsc{first} condition}
%     \begin{tabular}{lrrrrrr}
%       \hline
%       {\bf Setting} & {\bf Tratz} & {\bf \oshay Coarse} & {\bf \oshay Dir.} & {\bf \oshay Fine} & {\bf Kim\&Baldwin}  & {\bf Wordrobe} \\
%       \hline
%       \textsc{original} & $79.4$ $(0.0)$ & $62.3$ $(0.9)$ & $58.8$ $(1.1)$ & $50.9$ $(0.6)$ & $52.5$ $(0.4)$ & $54.2$ $(3.0)$ \\
%       \textsc{ppdb s} & $0.612$ $(0.0)$ & $0.585$  & $0.502$ & $0.786$\\
%       \textsc{ppdb m} & $0.619$ $(0.0)$ & $0.588$ & $0.491$ & $0.788$\\
%       \textsc{ppdb l} & $0.623$ $(0.0)$ & $0.602$ & $0.526$ & $0.784$\\
%       \textsc{ppdb xl} & $0.623$ $(0.0)$ & $0.571$ & $0.509$ & $0.785$ & $0.516$\\
%       \textsc{wn first} & $0.599$ $(0.0)$ & $0.564$ & $0.464$ & $0.782$ & $0.500$\\
%       \textsc{wn all} & $0.557$ $(0.0)$ & $0.519$ & $0.450$ & $0.762$ & $0.505$\\
%     \hline
%     \end{tabular}
%   \end{subtable}
%
%   \vspace{5mm}
%
%   \begin{subtable}{\textwidth}
%     \caption{\label{tab:last_dev_results}\textsc{last} condition}
%     \begin{tabular}{lrrrrrr}
%       \hline
%       {\bf Setting} & {\bf Tratz} & {\bf \oshay Coarse} & {\bf \oshay Dir.} & {\bf \oshay Fine} & {\bf Kim\&Baldwin}  & {\bf Wordrobe}\\
%       \hline
%       \textsc{original}  & $79.4$ $(0.0)$ & $62.3$ $(0.9)$ & $58.8$ $(1.1)$ & $50.9$ $(0.6)$ & $52.5$ $(0.4)$ & $\textbf{54.2}$ $(3.0)$ \\
%       \textsc{ppdb s} & $0.623$ & $0.599$ & $0.495$ & $0.787$\\
%       \textsc{ppdb m} & $0.623$ & $0.585$ & $0.502$ & $0.784$\\
%       \textsc{ppdb l} & $0.626$ & $0.595$ & $0.491$ & $0.786$ & $0.557$\\
%       \textsc{ppdb xl} & $0.616$ & $0.567$ & $0.471$ & $0.770$ & $0.500$\\
%       \textsc{wn first} & $0.592$ & $0.571$ & $0.460$ & $0.771$ & $0.521$\\
%       \textsc{wn all} & $0.550$ & $0.498$ & $0.408$ & $0.710$ & $0.526$\\
%     \hline
%     \end{tabular}
%   \end{subtable}
% \end{table*}

\section{Discussion}

\subsection{Dataset Augmentation for Animacy Classification}

In the case of animacy classification, although our system outperforms that of \citet{bowman:2012}, the results obtained are generally lower than those obtained in \citet{bjerva:14:eacl}.
This can be explained by several factors.

On the one hand, we can conclude that the proposed method for dataset augmentation does not work in the case of animacy classification.
This may be due to the fact that the animacy of a given entity is much more context dependant than the relation within a noun compound.
For instance, in the animacy scheme proposed by \citet{zaenen:2004}, entities should be annotated as \textsc{human} if they act in a human or human-like manner.
This means that in the case of, e.g., fables, in which animals speak as if they were human, the \textsc{human} tag should be assigned.
If we then add a number of training examples of paraphrases of various animals with this tag, and later encounter an animal in a different context, the chances of misclassifying this are high.

Another factor is the fact that the animacy dataset was much larger than the other supplied datasets.
It is possible that the already large dataset size does not lend itself to further dataset augmentation, as in the case of \citet{Zhang:2015}.

Due to the absence of differences in the animacy classification conditions, the rest of this chapter's discussion deals with the outcomes of the noun compound classification tasks.

\subsection{Comparing two lexical resources}

In this chapter, we compared the effects of using PPDB 2.0 as opposed to WordNet 3.0 for dataset augmentation.
For all cases, using PPDB yielded improved results as compared to WordNet.
This can be explained by several factors.
In order for dataset augmentation to be beneficial, it is essential that invariant properties of the dataset are varied (cf. Section~\ref{sec:dataset_augmentation_background}).
In the case of our approach, based on replacing words, and in the case of noun compound interpretation, this means that we wish to augment the dataset by replacing nouns with other closely related nouns, such that the semantic relation in the noun compound remains the same.

\subsubsection*{WordNet}
\noindent Augmenting datasets using WordNet synsets did not yield satisfactory results.
Two salient choices of either replacing words with lemmas from the most frequent synset of the word at hand, or with all lemmas of \textit{all} synsets of the word at hand resulted in the \textsc{wn first} and \textsc{wn all} settings.
This means that, in the \textsc{wn first} setting, the dataset is augmented by replacing words with (potentially wrong)\footnote{Potentially wrong is here meant to indicate that, depending on which WN sense is the first sense of a given word, an erroneous sense may be selected.} synonyms.
Similarly, in the \textsc{wn all} setting, words are replaced with both correct and erroneous synonyms.
Choosing correct augmentation examples is thus highly dependent on the correct choice of synsets, and the use of heuristics such as the aforementioned is likely to be problematic.
Indeed, in our WN augmentation settings, classification accuracy was lower than in the unaugmented settings, as evaluated in the cross-validation setting.
The fact that word-sense disambiguation is a very difficult task for which context is exceedingly important, and that datasets such as the ones used in this study provide very little context, further highlights the problems of using WN to this end.
These problems indicate that the resource is not particularly suited for dataset augmentation, which may explain the relatively small increase in system performance obtained by \citet{Zhang:2015}.

\subsubsection*{The Paraphrase Database}
\noindent Augmenting datasets using PPDB synonyms yielded substantial improvements when the entailment relations were used.
%Word senses are not encoded in PPDB, hence the problem of choosing the correct senses is bypassed in this resource.
The wide range of semantic relations present in the PPDB can be seen as a challenge for approaches such as dataset augmentation.
For instance, when augmenting an example with an \textsc{other-related} paraphrase, one does not expect the augmented example to maintain its noun compound semantic relation.
As an example, in the compound \textit{prison escape}, if \textit{prison} is replaced with the paraphrase \textit{prisoner} (\textsc{ppdb xl}), the compound relation changes from \textsc{object} to \textsc{subject}.
Using paraphrases for dataset augmentation may therefore seem less robust than using synonyms, as many paraphrases are subject to semantic drift, and can have quite different meanings (e.g. \textit{care} paraphrased as \textit{payload} (see Table~\ref{tab:augment_examples})).
However, with the recently released PPDB 2.0, the addition of explicit entailment relations appears to outweigh this drawback.
In the cross-validation setting, we compared results when including and excluding extra features based on these entailment relations, and found a consistent increase in performance when such features are included.
This means that, although the PPDB does not encode senses, and although paraphrases can have many types of semantic relations, such information is helpful for dataset augmentation.
The issue of semantic drift may further be countered by, e.g., filtering with a language model.
This was outside of the scope of this work and is currently being explored.

When augmenting datasets it is important to alter invariant properties of the data (cf. Section~\ref{sec:dataset_augmentation_background}).
The results shown here indicate that altering properties which are not invariant of the data is not necessarily detrimental to system performance, as long as this information is included as a feature (see Table~\ref{tab:entailment_results}).
Although beyond the scope of this work, it would be interesting to perform experiments with WordNet looking at whether including lemmas from relations of a given synset (e.g. \textit{cat}) such as hypernyms (e.g. \textit{feline}), hyponyms (e.g. \textit{siamese}) or co-hyponyms (e.g. \textit{dog}) would further aid performance.
The case of defining co-hyponyms would, however, be a challenge in itself, considering that these are not explicitly defined in WordNet and require constraints to be set in terms of how far removed the shared hypernym of two would-be co-hyponyms should be.
Such challenges further highlight the advantage of using PPDB for dataset augmentation, as such concerns are more simply covered by using different sizes of the PPDB.

\subsection{Replacement conditions}
Results from the cross-validation setting indicate that augmenting the datasets using either only \textsc{unigram} replacement or \textsc{unigram+bigram} replacement is beneficial.
This can be explained by the fact that \textsc{unigram} replacement represents a relatively mild form of dataset augmentation, as only a portion of the compound is altered and assumed to carry the same semantic relation.
In the case of \textsc{bigram} replacement, however, the compound as a whole is replaced.
Considering that this leads to examples such as \textit{office holder} (\textsc{objective}) being replaced with \textit{full member} (\textsc{ppdb xl}), this can be seen as a somewhat risky move.
Nonetheless, in conjunction with the entailment relation features, using \textsc{bigram+unigram} replacements at the same time leads to an increase in performance.
This can be explained by the fact that adding such questionable training examples increases the robustness and generalisation ability of the neural network.

\subsection{Error analysis}
An error analysis shows that our method of dataset augmentation generates augmented training examples with both correct and incorrect tags.
This, in turn, leads to certain instances in the testing data being classified correctly only in the augmented setting, while others are classified correctly only in the unaugmented setting.

For instance, the Tratz training set contains \textit{fox hunting} and \textit{deer hunting} (tagged \textsc{objective}).
In the \textsc{PPDB S} condition, these are paraphrased to \textit{fox hunt} and \textit{deer hunt}, and can be considered successful augmentation examples.
This is further supported by the fact that the test set instance \textit{witch hunt} is only classified correctly when using dataset augmentation.
A negative example can be found where \textit{skiing championship} is paraphrased as \textit{ski championship} (tagged \textsc{perform\&engage in}).
In the test data, the instance \textit{ski promotion} is consequently only correctly classified in the unaugmented setting.

\subsection{Dataset dependent results}

\subsubsection*{\citet{Tratz:2011} dataset}
\noindent The results presented on the Tratz dataset in this chapter outperform the highest results found in the literature \citep{DimaHinrichs:2015,TratzHovy:2010}.
Interestingly, \citet{DimaHinrichs:2015} use a similar approach to our own, with the exception of dataset augmentation techniques, and report far lower accuracies when using the same precomputed word2vec embeddings.
This can be explained by the fact that the neural network setup used in their work does not include recent advances such as \mbox{ReLUs}, maxout or dropout, all of which are significant aids to training deep neural networks in general, and were found to yield higher classification accuracies on preliminary experiments in this work.
Hence, the improved \textit{unaugmented} performance on the test set as compared to \citet{DimaHinrichs:2015} can be accounted for by looking at architectural choices.
Furthermore, adding dataset augmentation results in outperforming all of their settings.

\subsubsection*{\citet{Oseaghdha:2008} dataset}
\noindent On the \oshay dataset, our results are generally lower than those reported in the literature.
This can partially be explained by the fact that \citet{OseaghdhaCopestake:2013} use fewer labels in their study, as they exclude labels occuring 10 times or fewer.
Furthermore, the features used in their system are quite sophisticated.
This indicates a potential drawback of using only word embeddings for this task, and highlights the need of using more linguistic information.
Nonetheless, a comparison of the unaugmented and augmented settings on the test sets revealed slight improvements when using dataset augmentation for the Coarse and Directed subsets.
As for the Fine subset, smaller differences were observed.
This can be explained by the fact that the tags in this subset are very fine-grained and stem from certain annotation rules.
Replacing words with \mbox{(near-)synonyms} is therefore quite likely to be wrong.
Even though such replacements can be said to convey the same noun compound semantic relation, they may not be correct in the case of rule selection for annotation.

\subsubsection*{\citet{KimBaldwin:2005} dataset}
\noindent On the Kim \& Baldwin dataset, some improvement was observed when using dataset augmentation in the cross-validation and test settings.

\subsubsection*{Wordrobe dataset}
\noindent The results presented for the Wordrobe dataset are in line with those reported for the other datasets, with some improvement observed when using dataset augmentation in cross-validation and test settings.
This also constitutes the first published results using this dataset.

% \subsection{Generality}
% How general is this dataset augmentation method?
% Can it be extended to other tasks?
% Noun compounds certainly lend themselves very nicely to this approach.

% \subsection{Improvement beyond the state-of-the-art}
%
% The procedure outlined in this chapter resulted in improved performance as compared to a baseline system on all datasets, and state-of-the-art performance on some datasets.
% Tuning various aspects of the learning architecture and using more sophisticated features would increase the classification performance further, likely outperforming the current state-of-the-art.
% Training task-specific word embeddings and adding in linguistically motivated features, as done by e.g. \citet{OseaghdhaCopestake:2013}, would be a suitable first step in this direction.

% \subsection{Other languages}
% PPDB available in 23 languages \citep{ppdb:multilingual}.
% WN available in over 200 languages \citep{wn:universal}.


\section{Conclusions and Future Work}
We have shown that dataset augmentation can be applied to noun compound classification with performance gains upon unaugmented baselines.
Furthermore, state-of-the-art performances were obtained for one of the four datasets, even though our main goal was not to outperform previous approaches (we used only a set of easily obtained features).
However, applying dataset augmentation to the task of animacy classification did not prove fruitful.
Given the evident advantages and challenges of augmenting linguistic datasets, future work should investigate the possibilities of applying this method or develop other methods for dataset augmentation for other linguistic classification tasks such as semantic role labelling and co-reference resolution.
Expanding on our ideas may lead to a general dataset augmentation method for NLP, thus increasing system performance for a large number of applications.
%In doing so, one could investigate whether the benefits of \mbox{(near-)synonym} replacement is limited to semantic tasks.
%As the PPDB exists for several languages, future work should also attempt to apply this method to other languages.


==> comp_sem/neural_network.tex <==

\def\layersep{2.5cm}
\begin{tikzpicture}[scale=0.5,shorten >=1pt,->,draw=black!50, node distance=\layersep]
    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{neuron}=[circle,fill=black!25,minimum size=17pt,inner sep=0pt]
    \tikzstyle{constituent}=[neuron, fill=taskyblue];
    \tikzstyle{input neuron}=[neuron, fill=ta2skyblue];
    \tikzstyle{output neuron}=[neuron, fill=ta2scarletred];
    \tikzstyle{hidden neuron}=[neuron, fill=ta2orange];
    \tikzstyle{annot} = [text width=4em, text centered]

    % Draw the input layer nodes
    \foreach \name / \y in {1,...,2}
    % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
        \node[constituent, pin=left:{\scriptsize Const. \#\y}] (L-\name) at (-\layersep,-\y-1) {};

    % Draw the input layer nodes
    \foreach \name / \y in {1,...,4}
    % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
        \node[input neuron] (I-\name) at (0,-\y) {};

    % Draw the hidden layer nodes
    \foreach \name / \y in {1,...,4}
        \path[yshift=0cm]
            node[hidden neuron] (H-\name) at (\layersep,-\y cm) {};

    % Draw the output layer node
    \foreach \name / \y in {1,...,3}
        \path[yshift=-0.5cm]
            node[output neuron] (O-\name) at (5cm,-\y cm) {};
            %\node[output neuron,pin={[pin edge={->}]right:Output}, right of=H-3] (O) {};


    \foreach \dest in {1,...,2}
        \path (L-1) edge (I-\dest);
    \foreach \dest in {3,...,4}
        \path (L-2) edge (I-\dest);

    % Connect every node in the input layer with every node in the
    % hidden layer.
    \foreach \source in {1,...,4}
        \foreach \dest in {1,...,4}
            \path (I-\source) edge (H-\dest);

    % Connect every node in the hidden layer with the output layer
    \foreach \source in {1,...,4}
        \foreach \dest in {1,...,3}
            \path (H-\source) edge (O-\dest);

    % Annotate the layers
    \node[annot,above of=L-1, node distance=1cm] (nn) {\scriptsize Comp.\\ $n=2$};
    \node[annot,above of=H-1, node distance=1cm] (hl) {\scriptsize Hidden $n=600$};
    \node[annot,left of=hl,xshift=1.3cm] {\scriptsize Input $n=600$};
    \node[annot,right of=hl,xshift=-1.3cm] {\scriptsize Output $n=k$};
    \node[annot,right of=O-2,xshift=-2.1cm] { }; %Better centering
\end{tikzpicture}


==> frontmatter/quote.tex <==
test


==> frontmatter/to.tex <==
\thispagestyle{empty}

\begin{center}
        \vspace*{10pt}
        %\textit{To my wife, Noortje}

        \vspace*{30pt}
        %\textit{Foar Heit en Mem}
\end{center}


==> intro/abstract.tex <==
%\setcounter{chapter}{-1}
\chapter[Abstract]{}
\vspace{-3cm}
\begin{abstract}
    \footnotesize
\absprelude
%\emph{
In Natural Language Processing (NLP), we are generally concerned with the automatic analysis of natural language, often with the goal of solving a particular natural language task.
The traditional approach is to consider a single task for a single language at a time.
%For instance, considerable time and effort might be put into engineering a system solely for part-of-speech (POS) tagging of English.
However, neural networks are particularly well suited for broadening this approach, by considering data for multiple tasks and languages simultaneously, and have become one of the most popular techniques in NLP in recent years.
This is an important approach to explore further, as the key to improving the reliability of NLP, especially for low-resource languages, is to take advantage of all relevant data, whenever possible.
In \textbf{Part I} of this thesis, we begin with going through a crash-course in (deep) neural networks with a focus on NLP (Chapter 2).
We will then look at some ways in which neural networks can consider multiple tasks and languages at the same time (Chapter 3).
Specifically, we will consider multitask learning (MTL), and several common multilingual approaches.
%Such approaches rely on the fact that many NLP tasks are highly related.
%In the case of looking at other tasks, this relies on the fact that many NLP tasks exhibit high correlations with each other.
%This begs the question of how this fact can be exploited in order to improve NLP, as it is a colossal waste not to consider using data which shares similarities with the task in which one is interested.
%}

%\emph{
In \textbf{Part II} of this thesis, I look at exploiting the fact that many NLP tasks are highly related to one another.
This is done by experimenting with MTL using hard parameter sharing, which has proven beneficial for a variety of NLP tasks.
In spite of such successes, however, it is not clear \textit{when} or \textit{why} MTL is beneficial in NLP.
Chapter 4 contains a case study in which semantic tagging is shown to be beneficial for POS tagging.
This further highlights the question of when MTL is beneficial in NLP tagging tasks, which is explored using information-theoretic measures in Chapter 5.
%} % -- this denotes  part of the focus of this thesis.

%\emph{
Multilingual models can leverage the fact that many languages share commonalities with one another.
These resemblances can occur on various levels, with languages sharing, for instance, syntactic, morphological, or lexical features.
%Such similarities can have many different causes, such as common language ancestry, loan words, or being a result of constraints in the properties of natural language itself.
%As in the case of related NLP tasks, this begs the question of how multilinguality can be exploited in order to improve NLP, as it is also a colossal waste not to consider using, e.g., Norwegian POS data when training a Danish POS tagger.
While there are many possibilities for exploiting these commonalities, the focus in this thesis is on using multilingual word representations, as they allow for straight-forward integration in a neural network.
As with MTL, it is not clear in which cases it is an advantage to \textit{go multilingual}.
In \textbf{Part III}, I begin with presenting a case study on multilingual semantic textual similarity (Chapter 6).
Following this, I explore how similar languages need to be, and in which way, in order to for it to be useful to go multilingual (Chapter 7).
%}

%\emph{
In \textbf{Part IV} of this thesis, I experiment with a combined paradigm, in which a neural network is trained on several languages and tasks simultaneously (Chapter 8).
%Additionally, the related concept of dataset augmentation is explored, with the goal of enhancing lexical NLP system performance on a general level.
Finally, the thesis is concluded in \textbf{Part V} (Chapter 9).
The experiments in this thesis are run on a large collection of mainly lexically oriented tasks, both semantic and morphosyntactic in nature, and on a total of 60 languages, representing a relatively wide typological range.
%}

\end{abstract}


==> listofitems.tex <==
% Ce fichier contient le code de l'extension "listofitems"
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
\def\loiname                 {listofitems}                           %
\def\loiver                      {1.4}                               %
%                                                                    %
\def\loidate                  {2017/10/05}                           %
%                                                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% --------------------------------------------------------------------
% Author     : Christian Tellechea, Steven B. Segletes
% Status     : Maintained
% Maintainer : Christian Tellechea
% Email      : unbonpetit@netc.fr
%              steven.b.segletes.civ@mail.mil
% Package URL: https://www.ctan.org/pkg/listofitems
% Bug tracker: https://framagit.org/unbonpetit/listofitems/issues
% Repository : https://framagit.org/unbonpetit/listofitems/tree/master
% Copyright  : Christian Tellechea 2017
% Licence    : Released under the LaTeX Project Public License v1.3c
%              or later, see http://www.latex-project.org/lppl.txt
% Files      : 1) listofitems.tex
%              2) listofitems.sty
%              3) listofitems-fr.tex
%              4) listofitems-fr.pdf
%              5) listofitems-en.tex
%              6) listofitems-en.pdf
%              7) README
% --------------------------------------------------------------------
\expandafter\edef\csname loi_restorecatcode\endcsname{\catcode\number`\_=\number\catcode`\_\relax}
\catcode`\_11

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% gestion des erreurs %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifdefined\PackageError
	\def\loi_error#1{\PackageError\loiname{#1}{Read the manual}}% pour LaTeX
\else
	\def\loi_error#1{\errmessage{Package \loiname\space Error: #1^^J}}% pour TeX
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% v\'erification de la pr`'esence de etex %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begingroup
\edef\__tempa{\meaning\eTeXversion}\edef\__tempb{\string\eTeXversion}%
\ifx\__tempa\__tempb
	\endgroup
\else
	\endgroup
	\loi_error{You are not using an eTeX engine, listofitems cannot work.}%
	\expandafter\loi_restorecatcode\expandafter\endinput
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macros auxiliaires %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%---- macros de d\'eveloppement et de manipulation d'arguments
\chardef\loi_stop=0
\def\loi_quark{\loi_quark}
\long\def\loi_identity#1{#1}
\def\loi_gobarg#1{}
\long\def\loi_first#1#2{#1}
\long\def\loi_second#1#2{#2}
\long\def\loi_firsttonil#1#2\_nil{#1}
\long\def\loi_antefi#1#2\fi{#2\fi#1}
\long\def\loi_exparg#1#2{\expandafter\loi_exparg_i\expandafter{#2}{#1}}% \loi_exparg{<a>}{<b>} devient <a>{<*b>}
\long\def\loi_exparg_i#1#2{#2{#1}}
\long\def\loi_expafter#1#2{\expandafter\loi_expafter_i\expandafter{#2}{#1}}% \loi_expafter{<a>}{<b>} devient <a><*b>
\long\def\loi_expafter_i#1#2{#2#1}
\def\loi_macroname{\loi_ifinrange\escapechar[[0:255]]{\expandafter\loi_gobarg}{}\string}
\def\loi_argcsname#1#{\loi_argcsname_i{#1}}
\def\loi_argcsname_i#1#2{\loi_expafter{#1}{\csname#2\endcsname}}

%--- macros de test
\long\def\loi_ifnum#1{\ifnum#1\expandafter\loi_first\else\expandafter\loi_second\fi}
\long\def\loi_ifx#1{\ifx#1\expandafter\loi_first\else\expandafter\loi_second\fi}
\long\def\loi_ifempty#1{\loi_exparg\loi_ifx{\expandafter\relax\detokenize{#1}\relax}}
\def\loi_ifstar#1#2{\def\loi_ifstar_i{\loi_ifx{*\loi_nxttok}{\loi_first{#1}}{#2}}\futurelet\loi_nxttok\loi_ifstar_i}
\long\def\loi_ifprimitive#1{\edef\loi_tempa{\meaning#1}\edef\loi_tempb{\string#1}\loi_ifx{\loi_tempa\loi_tempb}}
\long\def\loi_ifcs#1{% #1 est-il une sc (n'\'etant pas une primitive) ?
	\loi_ifempty{#1}
		\loi_second% si #1 est vide, faux
		{\loi_ifspacefirst{#1}
			\loi_second% si espace en 1er, faux
			{\loi_exparg\loi_ifempty{\loi_gobarg#1}% 1 seul token ?
				{\begingroup \escapechar`\_
					\if\expandafter\loi_firsttonil\string#1\_nil\expandafter\loi_firsttonil\string\relax\_nil
						\loi_ifprimitive
							{\endgroup\expandafter\loi_second}
							{\endgroup\expandafter\loi_first}%
					\else
						\endgroup\expandafter\loi_second
					\fi
				}
				\loi_second% si plusieurs tokens, faux
			}%
		}%
}
\def\loi_ifinrange#1[[#2:#3]]{\loi_ifnum{\numexpr(#1-#2)*(#1-#3)>0 }\loi_second\loi_first}

%--- macro de type for
%      Voir codes 150 \`a 155 ici --> http://progtex.fr/wp-content/uploads/2014/09/code.txt
%      et pages 175 \`a 184 du livre "Apprendre \`a programmer en TeX"
\def\loi_fornum#1=#2to#3\do{%
	\edef#1{\number\numexpr#2}\edef\loi_sgncmp{\ifnum#1<\numexpr#3\relax>+\else<-\fi}%
	\expandafter\loi_fornum_i\csname loi_fornum_\string#1\expandafter\endcsname\expandafter{\number\numexpr#3\expandafter}\loi_sgncmp#1%
}
\long\def\loi_fornum_i#1#2#3#4#5#6{\def#1{\unless\ifnum#5#3#2\relax\loi_antefi{#6\edef#5{\number\numexpr#5#41\relax}#1}\fi}#1}

%--- macros retirant les espaces extr\^emes
%      Voir codes 320 \`a 324 ici --> http://progtex.fr/wp-content/uploads/2014/09/code.txt
%      et pages 339 \`a 343 de "Apprendre \`a programmer en TeX"
\long\def\loi_ifspacefirst#1{\expandafter\loi_ifspacefirst_i\detokenize{#10} \_nil}
\long\def\loi_ifspacefirst_i#1 #2\_nil{\loi_ifempty{#1}}
\expandafter\def\expandafter\loi_gobspace\space{}
\def\loi_removefirstspaces{\romannumeral\loi_removefirstspaces_i}
\long\def\loi_removefirstspaces_i#1{\loi_ifspacefirst{#1}{\expandafter\loi_removefirstspaces_i\expandafter{\loi_gobspace#1}}{\loi_stop#1}}
\edef\loi_restorezerocatcode{\catcode0=\number\catcode0 \relax}
\catcode0 12
\long\def\loi_removelastspaces#1{\romannumeral\loi_removelastspaces_i#1^^00 ^^00\_nil}
\long\def\loi_removelastspaces_i#1 ^^00{\loi_removelastspaces_ii#1^^00}
\long\def\loi_removelastspaces_ii#1^^00#2\_nil{\loi_ifspacefirst{#2}{\loi_removelastspaces_i#1^^00 ^^00\_nil}{\loi_stop#1}}
\loi_restorezerocatcode
\long\def\loi_removeextremespaces#1{% #1=texte o\`u les espaces extr\^emes sont retir\'es
	\romannumeral\expandafter\expandafter\expandafter\loi_removelastspaces\expandafter\expandafter\expandafter
	{\expandafter\expandafter\expandafter\loi_stop\loi_removefirstspaces{#1}}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% macro publique \setsepchar %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\setsepchar{\futurelet\loi_nxttok\setsepchar_i}
\def\setsepchar_i{\loi_ifx{[\loi_nxttok}\setsepchar_ii{\setsepchar_ii[/]}}
\long\def\setsepchar_ii[#1]#2{% #1=sepcar de <liste des sepcar>  #2=<liste des sepcar>
	\loi_ifempty{#1}
		{\loi_error{Empty separator not allowed, separator "/" used}%
		\setsepchar_ii[/]{#2}%
		}
		{\def\loi_currentsep{#1}%
		\_removeextremespacesfalse
		\loi_nestcnt1 % r\'einitaliser niveau initial \`a 1
		\def\nestdepth{1}%
		\loi_argcsname\let{loi_previndex[\number\loi_nestcnt]}\empty
		\def\loi_listname{loi_listofsep}%
		\let\loi_def\def \let\loi_edef\edef \let\loi_let\let
		\loi_ifempty{#2}
			{\loi_error{Empty list of separators not allowed, "," used}%
			\readlist_iv1{,}%
			}
			{\readlist_iv1{#2}}%
		\loi_argcsname\let\nestdepth{loi_listofseplen[0]}%
		\loi_argcsname\let\loi_currentsep{loi_listofsep[1]}% 1er car de s\'eparation
		}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% macro normalisant l'index %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\loi_normalizeindex#1#2#3{% #1=macroname  #2=liste d'index  #3=profondeur max --> renvoie {err}{indx norm}
	\loi_ifempty{#2}
		{\loi_stop{}{}}
		{\loi_normalizeindex_i1{}{#3}{#1}#2,\loi_quark,}%
}%
\def\loi_normalizeindex_i#1#2#3#4#5,{% #1=compteur de profondeur #2=index pr\'ec\'edents  #3=profondeur max #4=macroname  #5=index courant
	\loi_ifx{\loi_quark#5}
		{\loi_normalizeindex_iii#2\loi_quark}% supprimer la derni\`ere virgule
		{\loi_ifnum{#1>#3 }
			{\loi_invalidindex{Too deeply nested index, index [.] retained}{#2}}% si profondeur trop grande
			{\loi_ifinrange\ifnum\numexpr#5<0 -1*\fi(#5)[[1:\csname #4len[#20]\endcsname]]% si abs(#5) hors de [1,len]
				{\loi_exparg\loi_normalizeindex_ii{\number\numexpr#5\ifnum\numexpr#5<0 +\csname #4len[#20]\endcsname+1\fi}{#1}{#2}{#3}{#4}}
				{\loi_invalidindex{#5 is an invalid index, index [.] retained}{#2}}%
			}%
		}%
}
\def\loi_normalizeindex_ii#1#2#3{\loi_exparg\loi_normalizeindex_i{\number\numexpr#2+1}{#3#1,}}% #1=index \`a rajouter  #2=compteur de profondeur #3=index pr\'ec\'edents
\def\loi_normalizeindex_iii#1,\loi_quark{\loi_stop{}{#1}}
\def\loi_invalidindex#1#2{\loi_ifempty{#2}{\loi_invalidindex_i{#1},}\loi_invalidindex_i{#1}{#2}}
\def\loi_invalidindex_i#1#2{\loi_invalidindex_ii#1\loi_quark#2\loi_quark}
\def\loi_invalidindex_ii#1[.]#2\loi_quark#3,\loi_quark#4\loi_quark,{\loi_stop{#1[#3]#2}{#3}}% #4= index ignor\'es

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%% macro publique \readlist %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcount\loi_nestcnt
\def\greadlist{%
	\let\loi_def\gdef \let\loi_edef\xdef \def\loi_let{\global\let}%
	\loi_nestcnt1 % niveau initial = 1
	\loi_argcsname\loi_let{loi_previndex[\number\loi_nestcnt]}\empty
	\loi_ifstar{\_removeextremespacestrue\readlist_i}{\_removeextremespacesfalse\readlist_i}%
}
\def\readlist{%
	\let\loi_def\def \let\loi_edef\edef \let\loi_let\let
	\loi_nestcnt1 % niveau initial = 1
	\loi_argcsname\let{loi_previndex[\number\loi_nestcnt]}\empty
	\loi_ifstar{\_removeextremespacestrue\readlist_i}{\_removeextremespacesfalse\readlist_i}%
}
\long\def\readlist_i#1#2{% #1=macro stockant les \'el\'ements  #2=liste des \'el\'ements
	\loi_ifcs{#2}
		{\loi_exparg{\readlist_i#1}{#2}}
		{\loi_edef\loi_listname{\loi_macroname#1}%
		\loi_argcsname\loi_let{\loi_listname nest}\nestdepth
		\loi_argcsname\loi_def{\loi_listname[]}{#2}% la liste enti\`ere
		\loi_argcsname\loi_def{\loi_listname sep[]}{}% s\'eparateur vide
		\loi_ifempty{#2}
			{\loi_def#1[##1]{}%
			\loi_argcsname\loi_def{\loi_listname len}{0}\loi_argcsname\loi_def{\loi_listname len[0]}{0}%
			\loi_error{Empty list ignored, nothing to do}%
			}
			{\loi_edef#1[##1]{\unexpanded{\romannumeral\expandafter\loi_auxmacrolistitem\romannumeral\loi_normalizeindex}{\loi_listname}{##1}{\csname\loi_listname nest\endcsname}{\loi_listname}}%
			\loi_argcsname\loi_edef{\loi_listname sep}[##1]{\unexpanded{\romannumeral\expandafter\loi_auxmacrolistitem\romannumeral\loi_normalizeindex}{\loi_listname}{##1}{\csname\loi_listname nest\endcsname}{\loi_listname sep}}%
			\readlist_ii{#2}%
			\loi_argcsname\loi_argcsname\loi_let{\loi_listname len}{\loi_listname len[0]}% longueur du niveau 0
			}%
		}%
}
\def\loi_auxmacrolistitem#1#2#3{%
	\expandafter\expandafter\expandafter\loi_stop\csname#3[#2]\expandafter\endcsname
	\romannumeral\loi_ifempty{#1}{\loi_stop}{\loi_stop\loi_error{#1}}%
}
\def\readlist_ii{%
	\loi_argcsname\loi_let\loi_currentsep{loi_listofsep[\number\loi_nestcnt]}%
	\expandafter\readlist_iii\loi_currentsep||\_nil
}
\long\def\readlist_iii#1||#2\_nil#3{\readlist_iv1{#3#1}}% #1=<sep courant simple>  #3=liste -> rajoute un \'el\'ement vide pour le test ifempty ci dessous
\long\def\readlist_iv#1#2{% #1=compteur d'index  #2=liste d'\'el\'ements \`a examiner
	\loi_ifempty{#2}
		{\loi_argcsname\loi_edef{\loi_listname len[\csname loi_previndex[\number\loi_nestcnt]\endcsname0]}{\number\numexpr#1-1\relax}%
		\advance\loi_nestcnt-1
		\loi_argcsname\loi_let\loi_currentsep{loi_listofsep[\number\loi_nestcnt]}%
		}
		{\loi_expafter{\readlist_vi{#2}{}}\loi_currentsep||\loi_quark||#2\_nil{#1}}% aller isoler le 1er item
}
\long\def\readlist_v#1#2{\readlist_vi{#2}{}#1||\loi_quark||#2\_nil}% #1=liste s\'eparateurs (s\'ep=||)  #2=chaine de tokens
\long\def\readlist_vi#1#2#3||{% #1=liste restante   #2=dernier <sep utile>  #3=<sep courant>
	\loi_ifx{\loi_quark#3}
		{\loi_ifempty{#2}% si #1 vide, aucun <sep utile> n'a \'et\'e trouv\'e, il reste \`a lire "<liste compl\`ete>\_nil"
			{\long\def\readlist_vii##1\_nil##2{\loi_exparg{\readlist_ix{##2}{}}{\loi_gobarg##1}{#2}}}% ##2=compteur d'index
			{\long\def\readlist_vii##1#2{\loi_exparg\readlist_viii{\loi_gobarg##1}\relax}%
			\long\def\readlist_viii##1##2\_nil##3{\loi_exparg{\readlist_ix{##3}}{\loi_gobarg##2}{##1}{#2}}% ##3=compteur d'index
			}%
		\readlist_vii\relax% le \relax meuble l'argument d\'elimit\'e
		}
		{\long\def\readlist_vii##1#3##2\_nil{%
			\loi_ifempty{##2}% si <liste restante> ne contient pas le <sep courant>
				{\readlist_vi{#1}{#2}}% recommencer avec le m\^eme <sep utile>
				{\readlist_vi{##1#3}{#3}}% sinon raccourcir <liste restante> et <sep courant>:=<sep utile>
			}%
		\readlist_vii#1#3\_nil
		}%
}
\long\def\readlist_ix#1#2#3{% #1=compteur d'index  #2=liste restante  #3=\'el\'ement courant
	\loi_ifnum{0\loi_exparg\loi_ifspacefirst{\loi_currentsep}{}1\if_removeextremespaces1\fi=11 }% s'il faur retirer les espaces extr\^emes
		{\loi_exparg{\loi_exparg{\readlist_x{#1}{#2}}}{\loi_removeextremespaces{#3}}}% red\'efinir l'\'el\'ement courant
		{\readlist_x{#1}{#2}{#3}}%
}
\long\def\readlist_x#1#2#3#4{% #1=compteur d'index  #2=liste restante  #3=\'el\'ement courant   #4=sep utilis\'e
	\loi_ifnum{0\if_ignoreemptyitems1\fi\loi_ifempty{#3}1{}=11 }
		{\readlist_iv{#1}{#2}}% si l'on n'ignore pas les \'el\'ements vides :
		{\loi_argcsname\loi_def{\loi_listname[\csname loi_previndex[\number\loi_nestcnt]\endcsname#1]}{#3}% assignation de l'item ctuel \`a la macro
		\loi_argcsname\loi_def{\loi_listname sep[\csname loi_previndex[\number\loi_nestcnt]\endcsname#1]}{#4}% assignation du <sep> actuel \`a la macro \<macrolist>sep
		\loi_ifnum{\loi_nestcnt<\nestdepth\relax}% si imbrication max non atteinte
			{\advance\loi_nestcnt1
			\loi_argcsname\edef{loi_previndex[\number\loi_nestcnt]}{\csname loi_previndex[\number\numexpr\loi_nestcnt-1]\endcsname#1,}%
			\readlist_ii{#3}% recommencer avec l'\'el\'ement courant
			}
			{}%
		\loi_exparg\readlist_iv{\number\numexpr#1+1}{#2}% puis chercher l'\'el\'ement suivant dans la liste restante
		}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%% macro \listlen %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\listlen#1[#2]{%
	\romannumeral\loi_ifempty{#2}
		{\expandafter\expandafter\expandafter\loi_stop\csname\loi_macroname#1len[0]\endcsname}
		{\loi_exparg\listlen_i{\romannumeral-`\.\loi_macroname#1}{#2}}%
}
\def\listlen_i#1#2{% #1=macro name   #2=index non normalis\'e    prendre <profondeur max-1>
	\loi_exparg{\expandafter\listlen_ii\romannumeral\loi_normalizeindex{#1}{#2}}{\number\numexpr\csname#1nest\endcsname-1}{#1}%
}
\def\listlen_ii#1#2#3{% #1=err   #2=index normalis\'e  #3=macroname
	\expandafter\expandafter\expandafter\loi_stop\csname#3len[#2,0]\expandafter\endcsname
	\romannumeral\loi_ifempty{#1}{\loi_stop}{\loi_stop\loi_error{#1}}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macro \foreachitem %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\foreachitem#1\in#2{%
	\edef\foreachitem_i{\noexpand\foreachitem_iii\noexpand#1{\expandafter\noexpand\csname\loi_macroname#1cnt\endcsname}{\loi_macroname#2}}%
	\futurelet\loi_nxttok\foreachitem_ii
}
\def\foreachitem_ii{\loi_ifx{\loi_nxttok[}\foreachitem_i{\foreachitem_i[]}}
\def\foreachitem_iii#1#2#3[#4]{% prendre <profondeur max-1>
	\loi_exparg{\expandafter\foreachitem_iv\romannumeral\loi_normalizeindex{#3}{#4}}{\number\numexpr\csname#3nest\endcsname-1}#1{#2}{#3}%
}
\def\foreachitem_iv#1#2{\loi_ifempty{#2}{\foreachitem_v{#1}{}}{\foreachitem_v{#1}{#2,}}}% #1=err  #2=index norm
\long\def\foreachitem_v#1#2#3#4#5#6{% #1=err  #2=index norm  #3=macroiter  #4=compteur associ\'e  #5=nom de macrolist  #6=code
	\loi_ifnum{\csname#5len[#20]\endcsname>0 }
		{\loi_ifempty{#1}{}{\loi_error{#1}}%
		\loi_fornum#4=1to\csname#5len[#20]\endcsname\do{\loi_argcsname\let#3{#5[#2#4]}#6}%
		}
		{}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%% macro \showitem %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\showitems{\loi_ifstar{\let\showitems_cmd\detokenize\showitems_i}{\let\showitems_cmd\loi_identity\showitems_i}}
\def\showitems_i#1{\def\showitems_ii{\showitems_iv#1}\futurelet\loi_nxttok\showitems_iii}
\def\showitems_iii{\loi_ifx{\loi_nxttok[}\showitems_ii{\showitems_ii[]}}
\def\showitems_iv#1[#2]{\foreachitem\showitems_iter\in#1[#2]{\showitemsmacro{\expandafter\showitems_cmd\expandafter{\showitems_iter}}}}
\unless\ifdefined\fbox
	\newdimen\fboxrule \newdimen\fboxsep \fboxrule=.4pt \fboxsep=3pt % r\'eglages identiques \`a LaTeX
	\def\fbox#1{% imitation de la macro \fbox de LaTeX, voir codes 251 \`a 254 ici --> http://progtex.fr/wp-content/uploads/2014/09/code.txt
		\hbox{% et pages 271 \`a 274 de "Apprendre \`a programmer en TeX"
			\vrule width\fboxrule
			\vtop{%
				\vbox{\hrule height\fboxrule \kern\fboxsep \hbox{\kern\fboxsep#1\kern\fboxsep}}%
				\kern\fboxsep \hrule height\fboxrule
			}\vrule width\fboxrule
		}%
	}
\fi
\def\showitemsmacro#1{% encadrement par d\'efaut
	\begingroup\fboxsep=0.25pt \fboxrule=0.5pt \fbox{\strut#1}\endgroup
	\hskip0.25em\relax
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macro \itemtomacro %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\itemtomacro#1[#2]{% #1[#2]=item  non encore lu: #3=macro
	\edef\loi_listname{\loi_macroname#1}%
	\loi_exparg{\expandafter\itemtomacro_i\romannumeral\expandafter\loi_normalizeindex\expandafter{\loi_listname}{#2}}{\csname\loi_listname nest\endcsname}\let
}
\def\gitemtomacro#1[#2]{% #1[#2]=item
	\xdef\loi_listname{\loi_macroname#1}%
	\loi_exparg{\expandafter\itemtomacro_i\romannumeral\expandafter\loi_normalizeindex\expandafter{\loi_listname}{#2}}{\csname\loi_listname nest\endcsname}{\global\let}%
}
\def\itemtomacro_i#1#2#3#4{%
	\loi_ifempty{#1}{}{\loi_error{#1}}%
	\loi_argcsname#3#4{\loi_listname[#2]}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%% r\'eglages par d\'efaut %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\if_removeextremespaces
\newif\if_ignoreemptyitems
\let\ignoreemptyitems\_ignoreemptyitemstrue
\let\reademptyitems\_ignoreemptyitemsfalse
\setsepchar{,}
\reademptyitems

\loi_restorecatcode
\endinput

######################################################################
#                             Historique                             #
######################################################################

v1.0  19/8/2016
      - Premi\`ere version publique

v1.1  01/09/2016
      - Stockage des s\'eparateurs dans <macrolist>sep
      - bug corrig\'e dans \loi_restorecatcode

v1.2  22/10/2016
      - macros \greadlist et \gitemtomacro pour la globalit\'e

v1.3  18/11/2016
      - bugs corrig\'es dans la gestion de la globalit\'e

v1.4  05/10/2017
      - test \loi_ifprimitive ajout\'e au test \loi_ifcs
      - suppression de \loi_expafternil, cr\'eation de \loi_expafter,
        modification de \loi_argcsname
      - correction d'un bug : \setsepchar{\par} ne provoque plus
        d'erreur. \loi_ifnum devient \long
